The Pan-STARRS1 Photometric System

The Pan-STARRS1 survey is collecting multi-epoch, multi-color observations of the sky north of declination -30 deg to unprecedented depths. These data are being photometrically and astrometrically calibrated and will serve as a reference for many other purposes. In this paper we present our determination of the Pan-STARRS photometric system: gp1, rp1, ip1, zp1, yp1, and wp1. The Pan-STARRS photometric system is fundamentally based on the HST Calspec spectrophotometric observations, which in turn are fundamentally based on models of white dwarf atmospheres. We define the Pan-STARRS magnitude system, and describe in detail our measurement of the system passbands, including both the instrumental sensitivity and atmospheric transmission functions. Byproducts, including transformations to other photometric systems, galactic extinction, and stellar locus are also provided. We close with a discussion of remaining systematic errors.

==> psphot_mrt.tex <==
% Machine readable complete version of table tab:bandpass
% This lists the cross-sections for each of the Pan-STARRS1 bandpasses
\begin{deluxetable}{rrrrrrrrrrr}
\tabletypesize{\scriptsize}
\tablecolumns{8}
\tablecaption{\PS\ bandpasses}
\tablehead{  
\colhead{Wavelength} & 
\colhead{{\it Open}} & 
\colhead{\gps} & 
\colhead{\rps} & 
\colhead{\ips} & 
\colhead{\zps} & 
\colhead{\yps} & 
\colhead{\wps} &
\colhead{Aero} &
\colhead{Ray} &
\colhead{Mol}\\
}
\startdata
 380 & 0.096 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.945 & 0.694 & 0.998\\
 381 & 0.099 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.945 & 0.697 & 0.999\\
 382 & 0.103 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.945 & 0.700 & 0.999\\
 383 & 0.106 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.945 & 0.703 & 1.000\\
 384 & 0.110 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.945 & 0.705 & 1.000\\
 385 & 0.113 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.945 & 0.708 & 1.000\\
 386 & 0.117 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.946 & 0.711 & 1.000\\
 387 & 0.121 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.946 & 0.713 & 1.000\\
 388 & 0.125 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.001 & 0.946 & 0.716 & 1.000\\
 389 & 0.129 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.946 & 0.718 & 1.000\\
 390 & 0.133 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.946 & 0.721 & 1.000\\
 391 & 0.137 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.946 & 0.723 & 1.000\\
 392 & 0.142 & 0.001 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.946 & 0.725 & 1.000\\
 393 & 0.146 & 0.002 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.947 & 0.728 & 1.000\\
 394 & 0.151 & 0.004 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.947 & 0.731 & 1.000\\
 395 & 0.156 & 0.007 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.947 & 0.733 & 1.000\\
 396 & 0.161 & 0.012 & 0.000 & 0.000 & 0.000 & 0.000 & 0.008 & 0.947 & 0.735 & 1.000\\
 397 & 0.166 & 0.021 & 0.000 & 0.000 & 0.000 & 0.000 & 0.010 & 0.947 & 0.738 & 1.000\\
 398 & 0.171 & 0.035 & 0.000 & 0.000 & 0.000 & 0.000 & 0.014 & 0.947 & 0.740 & 1.000\\
 399 & 0.176 & 0.053 & 0.000 & 0.000 & 0.000 & 0.000 & 0.021 & 0.947 & 0.742 & 1.000\\
 400 & 0.182 & 0.073 & 0.000 & 0.000 & 0.000 & 0.000 & 0.032 & 0.948 & 0.744 & 1.000\\
 401 & 0.188 & 0.096 & 0.000 & 0.000 & 0.000 & 0.000 & 0.049 & 0.948 & 0.746 & 1.000\\
 402 & 0.194 & 0.118 & 0.000 & 0.000 & 0.000 & 0.000 & 0.071 & 0.948 & 0.749 & 1.000\\
 403 & 0.199 & 0.135 & 0.000 & 0.000 & 0.000 & 0.000 & 0.096 & 0.948 & 0.751 & 1.000\\
 404 & 0.205 & 0.147 & 0.000 & 0.000 & 0.000 & 0.000 & 0.123 & 0.948 & 0.753 & 1.000\\
 405 & 0.210 & 0.157 & 0.000 & 0.000 & 0.000 & 0.000 & 0.148 & 0.948 & 0.755 & 1.000\\
 406 & 0.217 & 0.163 & 0.000 & 0.000 & 0.000 & 0.000 & 0.169 & 0.948 & 0.758 & 1.000\\
 407 & 0.223 & 0.167 & 0.000 & 0.000 & 0.000 & 0.000 & 0.186 & 0.948 & 0.760 & 1.000\\
 408 & 0.228 & 0.171 & 0.000 & 0.000 & 0.000 & 0.000 & 0.198 & 0.949 & 0.762 & 1.000\\
 409 & 0.235 & 0.175 & 0.000 & 0.000 & 0.000 & 0.000 & 0.208 & 0.949 & 0.764 & 1.000\\
 410 & 0.242 & 0.181 & 0.000 & 0.000 & 0.000 & 0.000 & 0.216 & 0.949 & 0.766 & 1.000\\
 411 & 0.248 & 0.186 & 0.000 & 0.000 & 0.000 & 0.000 & 0.223 & 0.949 & 0.768 & 1.000\\
 412 & 0.254 & 0.192 & 0.000 & 0.000 & 0.000 & 0.000 & 0.231 & 0.949 & 0.770 & 1.000\\
 413 & 0.261 & 0.199 & 0.000 & 0.000 & 0.000 & 0.000 & 0.240 & 0.949 & 0.772 & 1.000\\
 414 & 0.268 & 0.204 & 0.000 & 0.000 & 0.000 & 0.000 & 0.248 & 0.949 & 0.774 & 1.000\\
 415 & 0.276 & 0.206 & 0.000 & 0.000 & 0.000 & 0.000 & 0.257 & 0.949 & 0.776 & 1.000\\
 416 & 0.284 & 0.208 & 0.000 & 0.000 & 0.000 & 0.000 & 0.265 & 0.950 & 0.778 & 1.000\\
 417 & 0.291 & 0.211 & 0.000 & 0.000 & 0.000 & 0.000 & 0.272 & 0.950 & 0.780 & 1.000\\
 418 & 0.298 & 0.217 & 0.000 & 0.000 & 0.000 & 0.000 & 0.278 & 0.950 & 0.782 & 1.000\\
 419 & 0.305 & 0.225 & 0.000 & 0.000 & 0.000 & 0.000 & 0.284 & 0.950 & 0.784 & 1.000\\
 420 & 0.312 & 0.233 & 0.000 & 0.000 & 0.000 & 0.000 & 0.288 & 0.950 & 0.785 & 1.000\\
 421 & 0.318 & 0.240 & 0.000 & 0.000 & 0.000 & 0.000 & 0.293 & 0.950 & 0.787 & 1.000\\
 422 & 0.324 & 0.246 & 0.000 & 0.000 & 0.000 & 0.000 & 0.297 & 0.950 & 0.789 & 1.000\\
 423 & 0.331 & 0.249 & 0.000 & 0.000 & 0.000 & 0.000 & 0.303 & 0.950 & 0.791 & 1.000\\
 424 & 0.338 & 0.250 & 0.000 & 0.000 & 0.000 & 0.000 & 0.308 & 0.951 & 0.792 & 1.000\\
 425 & 0.344 & 0.250 & 0.000 & 0.000 & 0.000 & 0.000 & 0.315 & 0.951 & 0.794 & 1.000\\
 426 & 0.351 & 0.253 & 0.000 & 0.000 & 0.000 & 0.000 & 0.322 & 0.951 & 0.796 & 1.000\\
 427 & 0.356 & 0.259 & 0.000 & 0.000 & 0.000 & 0.000 & 0.328 & 0.951 & 0.798 & 1.000\\
 428 & 0.362 & 0.268 & 0.000 & 0.000 & 0.000 & 0.000 & 0.335 & 0.951 & 0.799 & 1.000\\
 429 & 0.368 & 0.277 & 0.000 & 0.000 & 0.000 & 0.000 & 0.342 & 0.951 & 0.801 & 1.000\\
 430 & 0.374 & 0.286 & 0.000 & 0.000 & 0.000 & 0.000 & 0.350 & 0.951 & 0.803 & 1.000\\
 431 & 0.380 & 0.295 & 0.000 & 0.000 & 0.000 & 0.000 & 0.358 & 0.951 & 0.804 & 1.000\\
 432 & 0.386 & 0.300 & 0.000 & 0.000 & 0.000 & 0.000 & 0.367 & 0.952 & 0.806 & 1.000\\
 433 & 0.392 & 0.302 & 0.000 & 0.000 & 0.000 & 0.000 & 0.375 & 0.952 & 0.808 & 0.999\\
 434 & 0.398 & 0.302 & 0.000 & 0.000 & 0.000 & 0.000 & 0.382 & 0.952 & 0.809 & 0.999\\
 435 & 0.403 & 0.304 & 0.000 & 0.000 & 0.000 & 0.000 & 0.389 & 0.952 & 0.810 & 0.999\\
 436 & 0.409 & 0.309 & 0.000 & 0.000 & 0.000 & 0.000 & 0.396 & 0.952 & 0.812 & 0.999\\
 437 & 0.415 & 0.316 & 0.000 & 0.000 & 0.000 & 0.000 & 0.402 & 0.952 & 0.815 & 0.999\\
 438 & 0.420 & 0.323 & 0.000 & 0.000 & 0.000 & 0.000 & 0.408 & 0.952 & 0.817 & 0.999\\
 439 & 0.425 & 0.330 & 0.000 & 0.000 & 0.000 & 0.000 & 0.411 & 0.952 & 0.817 & 0.999\\
 440 & 0.430 & 0.336 & 0.000 & 0.000 & 0.000 & 0.000 & 0.416 & 0.952 & 0.819 & 0.999\\
 441 & 0.436 & 0.340 & 0.000 & 0.000 & 0.000 & 0.000 & 0.421 & 0.953 & 0.821 & 0.999\\
 442 & 0.442 & 0.341 & 0.000 & 0.000 & 0.000 & 0.000 & 0.426 & 0.953 & 0.823 & 0.999\\
 443 & 0.447 & 0.342 & 0.000 & 0.000 & 0.000 & 0.000 & 0.430 & 0.953 & 0.824 & 0.998\\
 444 & 0.451 & 0.344 & 0.000 & 0.000 & 0.000 & 0.000 & 0.433 & 0.953 & 0.825 & 0.999\\
 445 & 0.455 & 0.348 & 0.000 & 0.000 & 0.000 & 0.000 & 0.437 & 0.953 & 0.826 & 0.999\\
 446 & 0.460 & 0.354 & 0.000 & 0.000 & 0.000 & 0.000 & 0.442 & 0.953 & 0.828 & 0.999\\
 447 & 0.465 & 0.361 & 0.000 & 0.000 & 0.000 & 0.000 & 0.446 & 0.953 & 0.830 & 0.999\\
 448 & 0.470 & 0.368 & 0.000 & 0.000 & 0.000 & 0.000 & 0.449 & 0.953 & 0.830 & 0.999\\
 449 & 0.474 & 0.374 & 0.000 & 0.000 & 0.000 & 0.000 & 0.453 & 0.953 & 0.832 & 0.999\\
 450 & 0.478 & 0.380 & 0.000 & 0.000 & 0.000 & 0.000 & 0.458 & 0.954 & 0.834 & 0.999\\
 451 & 0.482 & 0.386 & 0.000 & 0.000 & 0.000 & 0.000 & 0.462 & 0.954 & 0.835 & 0.999\\
 452 & 0.486 & 0.392 & 0.000 & 0.000 & 0.000 & 0.000 & 0.467 & 0.954 & 0.836 & 0.999\\
 453 & 0.490 & 0.396 & 0.000 & 0.000 & 0.000 & 0.000 & 0.470 & 0.954 & 0.838 & 0.999\\
 454 & 0.493 & 0.398 & 0.000 & 0.000 & 0.000 & 0.000 & 0.473 & 0.954 & 0.839 & 0.999\\
 455 & 0.497 & 0.398 & 0.000 & 0.000 & 0.000 & 0.000 & 0.476 & 0.954 & 0.841 & 0.999\\
 456 & 0.500 & 0.394 & 0.000 & 0.000 & 0.000 & 0.000 & 0.480 & 0.954 & 0.842 & 0.998\\
 457 & 0.503 & 0.388 & 0.000 & 0.000 & 0.000 & 0.000 & 0.484 & 0.954 & 0.843 & 0.998\\
 458 & 0.506 & 0.384 & 0.000 & 0.000 & 0.000 & 0.000 & 0.488 & 0.954 & 0.844 & 0.998\\
 459 & 0.509 & 0.382 & 0.000 & 0.000 & 0.000 & 0.000 & 0.491 & 0.954 & 0.845 & 0.998\\
 460 & 0.512 & 0.384 & 0.000 & 0.000 & 0.000 & 0.000 & 0.494 & 0.955 & 0.847 & 0.997\\
 461 & 0.514 & 0.388 & 0.000 & 0.000 & 0.000 & 0.000 & 0.497 & 0.955 & 0.848 & 0.997\\
 462 & 0.517 & 0.393 & 0.000 & 0.000 & 0.000 & 0.000 & 0.500 & 0.955 & 0.849 & 0.997\\
 463 & 0.520 & 0.396 & 0.000 & 0.000 & 0.000 & 0.000 & 0.503 & 0.955 & 0.851 & 0.997\\
 464 & 0.521 & 0.396 & 0.000 & 0.000 & 0.000 & 0.000 & 0.507 & 0.955 & 0.851 & 0.997\\
 465 & 0.525 & 0.396 & 0.000 & 0.000 & 0.000 & 0.000 & 0.511 & 0.955 & 0.853 & 0.997\\
 466 & 0.528 & 0.397 & 0.000 & 0.000 & 0.000 & 0.000 & 0.515 & 0.955 & 0.855 & 0.997\\
 467 & 0.530 & 0.397 & 0.000 & 0.000 & 0.000 & 0.000 & 0.517 & 0.955 & 0.856 & 0.997\\
 468 & 0.532 & 0.399 & 0.000 & 0.000 & 0.000 & 0.000 & 0.518 & 0.955 & 0.856 & 0.997\\
 469 & 0.534 & 0.400 & 0.000 & 0.000 & 0.000 & 0.000 & 0.516 & 0.955 & 0.858 & 0.997\\
 470 & 0.537 & 0.401 & 0.000 & 0.000 & 0.000 & 0.000 & 0.512 & 0.956 & 0.859 & 0.996\\
 471 & 0.539 & 0.402 & 0.000 & 0.000 & 0.000 & 0.000 & 0.511 & 0.956 & 0.860 & 0.996\\
 472 & 0.541 & 0.403 & 0.000 & 0.000 & 0.000 & 0.000 & 0.511 & 0.956 & 0.861 & 0.996\\
 473 & 0.542 & 0.405 & 0.000 & 0.000 & 0.000 & 0.000 & 0.509 & 0.956 & 0.863 & 0.995\\
 474 & 0.543 & 0.408 & 0.000 & 0.000 & 0.000 & 0.000 & 0.506 & 0.956 & 0.863 & 0.995\\
 475 & 0.544 & 0.413 & 0.000 & 0.000 & 0.000 & 0.000 & 0.504 & 0.956 & 0.864 & 0.994\\
 476 & 0.545 & 0.418 & 0.000 & 0.000 & 0.000 & 0.000 & 0.503 & 0.956 & 0.866 & 0.992\\
 477 & 0.547 & 0.424 & 0.000 & 0.000 & 0.000 & 0.000 & 0.505 & 0.956 & 0.867 & 0.991\\
 478 & 0.548 & 0.431 & 0.000 & 0.000 & 0.000 & 0.000 & 0.510 & 0.956 & 0.868 & 0.991\\
 479 & 0.550 & 0.437 & 0.000 & 0.000 & 0.000 & 0.000 & 0.518 & 0.956 & 0.869 & 0.991\\
 480 & 0.552 & 0.441 & 0.000 & 0.000 & 0.000 & 0.000 & 0.526 & 0.957 & 0.870 & 0.992\\
 481 & 0.554 & 0.444 & 0.000 & 0.000 & 0.000 & 0.000 & 0.533 & 0.957 & 0.871 & 0.992\\
 482 & 0.555 & 0.446 & 0.000 & 0.000 & 0.000 & 0.000 & 0.538 & 0.957 & 0.872 & 0.992\\
 483 & 0.557 & 0.448 & 0.000 & 0.000 & 0.000 & 0.000 & 0.540 & 0.957 & 0.873 & 0.993\\
 484 & 0.558 & 0.451 & 0.000 & 0.000 & 0.000 & 0.000 & 0.542 & 0.957 & 0.874 & 0.993\\
 485 & 0.559 & 0.453 & 0.000 & 0.000 & 0.000 & 0.000 & 0.542 & 0.957 & 0.875 & 0.993\\
 486 & 0.561 & 0.456 & 0.000 & 0.000 & 0.000 & 0.000 & 0.542 & 0.957 & 0.876 & 0.994\\
 487 & 0.562 & 0.458 & 0.000 & 0.000 & 0.000 & 0.000 & 0.543 & 0.957 & 0.877 & 0.994\\
 488 & 0.564 & 0.460 & 0.000 & 0.000 & 0.000 & 0.000 & 0.546 & 0.957 & 0.878 & 0.994\\
 489 & 0.565 & 0.460 & 0.000 & 0.000 & 0.000 & 0.000 & 0.547 & 0.957 & 0.878 & 0.994\\
 490 & 0.567 & 0.459 & 0.000 & 0.000 & 0.000 & 0.000 & 0.550 & 0.957 & 0.880 & 0.993\\
 491 & 0.568 & 0.455 & 0.000 & 0.000 & 0.000 & 0.000 & 0.552 & 0.958 & 0.881 & 0.993\\
 492 & 0.570 & 0.451 & 0.000 & 0.000 & 0.000 & 0.000 & 0.553 & 0.958 & 0.882 & 0.993\\
 493 & 0.572 & 0.450 & 0.000 & 0.000 & 0.000 & 0.000 & 0.554 & 0.958 & 0.883 & 0.993\\
 494 & 0.574 & 0.453 & 0.000 & 0.000 & 0.000 & 0.000 & 0.555 & 0.958 & 0.883 & 0.993\\
 495 & 0.575 & 0.459 & 0.000 & 0.000 & 0.000 & 0.000 & 0.557 & 0.958 & 0.884 & 0.993\\
 496 & 0.577 & 0.463 & 0.000 & 0.000 & 0.000 & 0.000 & 0.559 & 0.958 & 0.885 & 0.992\\
 497 & 0.579 & 0.467 & 0.000 & 0.000 & 0.000 & 0.000 & 0.561 & 0.958 & 0.886 & 0.992\\
 498 & 0.581 & 0.471 & 0.000 & 0.000 & 0.000 & 0.000 & 0.562 & 0.958 & 0.887 & 0.991\\
 499 & 0.582 & 0.472 & 0.000 & 0.000 & 0.000 & 0.000 & 0.561 & 0.958 & 0.888 & 0.991\\
 500 & 0.582 & 0.471 & 0.000 & 0.000 & 0.000 & 0.000 & 0.559 & 0.958 & 0.889 & 0.990\\
 501 & 0.583 & 0.468 & 0.000 & 0.000 & 0.000 & 0.000 & 0.559 & 0.958 & 0.890 & 0.989\\
 502 & 0.584 & 0.466 & 0.000 & 0.000 & 0.000 & 0.000 & 0.561 & 0.958 & 0.891 & 0.988\\
 503 & 0.585 & 0.463 & 0.000 & 0.000 & 0.000 & 0.000 & 0.564 & 0.959 & 0.891 & 0.987\\
 504 & 0.587 & 0.459 & 0.000 & 0.000 & 0.000 & 0.000 & 0.567 & 0.959 & 0.892 & 0.986\\
 505 & 0.589 & 0.457 & 0.000 & 0.000 & 0.000 & 0.000 & 0.571 & 0.959 & 0.893 & 0.986\\
 506 & 0.591 & 0.456 & 0.000 & 0.000 & 0.000 & 0.000 & 0.573 & 0.959 & 0.894 & 0.986\\
 507 & 0.594 & 0.455 & 0.000 & 0.000 & 0.000 & 0.000 & 0.574 & 0.959 & 0.895 & 0.986\\
 508 & 0.596 & 0.456 & 0.000 & 0.000 & 0.000 & 0.000 & 0.575 & 0.959 & 0.896 & 0.986\\
 509 & 0.598 & 0.456 & 0.000 & 0.000 & 0.000 & 0.000 & 0.577 & 0.959 & 0.896 & 0.987\\
 510 & 0.601 & 0.457 & 0.000 & 0.000 & 0.000 & 0.000 & 0.580 & 0.959 & 0.897 & 0.987\\
 511 & 0.602 & 0.458 & 0.000 & 0.000 & 0.000 & 0.000 & 0.581 & 0.959 & 0.898 & 0.987\\
 512 & 0.604 & 0.459 & 0.000 & 0.000 & 0.000 & 0.000 & 0.583 & 0.959 & 0.899 & 0.987\\
 513 & 0.605 & 0.461 & 0.000 & 0.000 & 0.000 & 0.000 & 0.583 & 0.959 & 0.899 & 0.987\\
 514 & 0.607 & 0.465 & 0.000 & 0.000 & 0.000 & 0.000 & 0.582 & 0.959 & 0.900 & 0.987\\
 515 & 0.609 & 0.469 & 0.000 & 0.000 & 0.000 & 0.000 & 0.582 & 0.960 & 0.901 & 0.986\\
 516 & 0.611 & 0.473 & 0.000 & 0.000 & 0.000 & 0.000 & 0.582 & 0.960 & 0.902 & 0.986\\
 517 & 0.613 & 0.475 & 0.000 & 0.000 & 0.000 & 0.000 & 0.583 & 0.960 & 0.903 & 0.986\\
 518 & 0.615 & 0.476 & 0.000 & 0.000 & 0.000 & 0.000 & 0.586 & 0.960 & 0.904 & 0.985\\
 519 & 0.616 & 0.475 & 0.000 & 0.000 & 0.000 & 0.000 & 0.590 & 0.960 & 0.904 & 0.985\\
 520 & 0.617 & 0.473 & 0.000 & 0.000 & 0.000 & 0.000 & 0.594 & 0.960 & 0.905 & 0.985\\
 521 & 0.618 & 0.472 & 0.000 & 0.000 & 0.000 & 0.000 & 0.598 & 0.960 & 0.906 & 0.984\\
 522 & 0.620 & 0.473 & 0.000 & 0.000 & 0.000 & 0.000 & 0.602 & 0.960 & 0.906 & 0.984\\
 523 & 0.622 & 0.473 & 0.000 & 0.000 & 0.000 & 0.000 & 0.606 & 0.960 & 0.907 & 0.983\\
 524 & 0.624 & 0.474 & 0.000 & 0.000 & 0.000 & 0.000 & 0.609 & 0.960 & 0.908 & 0.982\\
 525 & 0.626 & 0.473 & 0.000 & 0.000 & 0.000 & 0.000 & 0.612 & 0.960 & 0.908 & 0.981\\
 526 & 0.627 & 0.472 & 0.000 & 0.000 & 0.000 & 0.000 & 0.615 & 0.960 & 0.909 & 0.980\\
 527 & 0.629 & 0.474 & 0.000 & 0.000 & 0.000 & 0.000 & 0.617 & 0.960 & 0.910 & 0.979\\
 528 & 0.630 & 0.477 & 0.000 & 0.000 & 0.000 & 0.000 & 0.619 & 0.961 & 0.910 & 0.978\\
 529 & 0.632 & 0.483 & 0.001 & 0.000 & 0.000 & 0.000 & 0.621 & 0.961 & 0.911 & 0.978\\
 530 & 0.634 & 0.489 & 0.001 & 0.000 & 0.000 & 0.000 & 0.623 & 0.961 & 0.912 & 0.977\\
 531 & 0.635 & 0.495 & 0.001 & 0.000 & 0.000 & 0.000 & 0.625 & 0.961 & 0.912 & 0.976\\
 532 & 0.637 & 0.498 & 0.001 & 0.000 & 0.000 & 0.000 & 0.627 & 0.961 & 0.913 & 0.976\\
 533 & 0.640 & 0.500 & 0.001 & 0.000 & 0.000 & 0.000 & 0.629 & 0.961 & 0.914 & 0.975\\
 534 & 0.643 & 0.501 & 0.002 & 0.000 & 0.000 & 0.000 & 0.631 & 0.961 & 0.914 & 0.975\\
 535 & 0.645 & 0.502 & 0.002 & 0.000 & 0.000 & 0.000 & 0.633 & 0.961 & 0.915 & 0.975\\
 536 & 0.647 & 0.502 & 0.003 & 0.000 & 0.000 & 0.000 & 0.635 & 0.961 & 0.916 & 0.976\\
 537 & 0.649 & 0.502 & 0.004 & 0.000 & 0.000 & 0.000 & 0.637 & 0.961 & 0.916 & 0.976\\
 538 & 0.651 & 0.502 & 0.005 & 0.000 & 0.000 & 0.000 & 0.639 & 0.961 & 0.917 & 0.976\\
 539 & 0.653 & 0.502 & 0.008 & 0.000 & 0.000 & 0.000 & 0.640 & 0.961 & 0.917 & 0.975\\
 540 & 0.654 & 0.501 & 0.011 & 0.000 & 0.000 & 0.000 & 0.641 & 0.961 & 0.918 & 0.975\\
 541 & 0.656 & 0.500 & 0.017 & 0.000 & 0.000 & 0.000 & 0.644 & 0.962 & 0.919 & 0.974\\
 542 & 0.659 & 0.496 & 0.026 & 0.000 & 0.000 & 0.000 & 0.647 & 0.962 & 0.919 & 0.974\\
 543 & 0.661 & 0.493 & 0.040 & 0.000 & 0.000 & 0.000 & 0.649 & 0.962 & 0.920 & 0.974\\
 544 & 0.663 & 0.489 & 0.062 & 0.000 & 0.000 & 0.000 & 0.651 & 0.962 & 0.920 & 0.973\\
 545 & 0.667 & 0.486 & 0.093 & 0.000 & 0.000 & 0.000 & 0.654 & 0.962 & 0.921 & 0.973\\
 546 & 0.670 & 0.481 & 0.134 & 0.000 & 0.000 & 0.000 & 0.656 & 0.962 & 0.921 & 0.972\\
 547 & 0.671 & 0.467 & 0.184 & 0.000 & 0.000 & 0.000 & 0.657 & 0.962 & 0.922 & 0.972\\
 548 & 0.672 & 0.438 & 0.242 & 0.000 & 0.000 & 0.000 & 0.658 & 0.962 & 0.923 & 0.972\\
 549 & 0.673 & 0.390 & 0.305 & 0.000 & 0.000 & 0.000 & 0.660 & 0.962 & 0.923 & 0.972\\
 550 & 0.675 & 0.323 & 0.367 & 0.000 & 0.000 & 0.000 & 0.662 & 0.962 & 0.924 & 0.971\\
 551 & 0.678 & 0.248 & 0.423 & 0.000 & 0.000 & 0.000 & 0.665 & 0.962 & 0.924 & 0.971\\
 552 & 0.682 & 0.175 & 0.469 & 0.000 & 0.000 & 0.000 & 0.668 & 0.962 & 0.925 & 0.971\\
 553 & 0.685 & 0.113 & 0.504 & 0.000 & 0.000 & 0.000 & 0.670 & 0.962 & 0.925 & 0.971\\
 554 & 0.688 & 0.068 & 0.528 & 0.000 & 0.000 & 0.000 & 0.672 & 0.963 & 0.926 & 0.970\\
 555 & 0.689 & 0.041 & 0.544 & 0.000 & 0.000 & 0.000 & 0.673 & 0.963 & 0.927 & 0.970\\
 556 & 0.690 & 0.025 & 0.556 & 0.000 & 0.000 & 0.000 & 0.674 & 0.963 & 0.927 & 0.969\\
 557 & 0.691 & 0.015 & 0.565 & 0.000 & 0.000 & 0.000 & 0.674 & 0.963 & 0.928 & 0.968\\
 558 & 0.691 & 0.009 & 0.570 & 0.000 & 0.000 & 0.000 & 0.675 & 0.963 & 0.928 & 0.968\\
 559 & 0.693 & 0.006 & 0.575 & 0.000 & 0.000 & 0.000 & 0.678 & 0.963 & 0.929 & 0.967\\
 560 & 0.695 & 0.003 & 0.578 & 0.000 & 0.000 & 0.000 & 0.680 & 0.963 & 0.929 & 0.966\\
 561 & 0.697 & 0.002 & 0.582 & 0.000 & 0.000 & 0.000 & 0.682 & 0.963 & 0.930 & 0.965\\
 562 & 0.699 & 0.002 & 0.584 & 0.000 & 0.000 & 0.000 & 0.683 & 0.963 & 0.930 & 0.964\\
 563 & 0.701 & 0.001 & 0.586 & 0.000 & 0.000 & 0.000 & 0.685 & 0.963 & 0.930 & 0.963\\
 564 & 0.703 & 0.001 & 0.588 & 0.000 & 0.000 & 0.000 & 0.686 & 0.963 & 0.931 & 0.962\\
 565 & 0.705 & 0.001 & 0.590 & 0.000 & 0.000 & 0.000 & 0.688 & 0.964 & 0.931 & 0.961\\
 566 & 0.707 & 0.001 & 0.591 & 0.000 & 0.000 & 0.000 & 0.690 & 0.964 & 0.932 & 0.961\\
 567 & 0.709 & 0.000 & 0.592 & 0.000 & 0.000 & 0.000 & 0.692 & 0.964 & 0.933 & 0.960\\
 568 & 0.710 & 0.000 & 0.592 & 0.000 & 0.000 & 0.000 & 0.695 & 0.964 & 0.933 & 0.958\\
 569 & 0.712 & 0.000 & 0.591 & 0.000 & 0.000 & 0.000 & 0.696 & 0.964 & 0.933 & 0.957\\
 570 & 0.714 & 0.000 & 0.591 & 0.000 & 0.000 & 0.000 & 0.698 & 0.964 & 0.934 & 0.956\\
 571 & 0.716 & 0.000 & 0.589 & 0.000 & 0.000 & 0.000 & 0.700 & 0.964 & 0.934 & 0.955\\
 572 & 0.717 & 0.000 & 0.586 & 0.000 & 0.000 & 0.000 & 0.700 & 0.964 & 0.935 & 0.954\\
 573 & 0.718 & 0.000 & 0.583 & 0.000 & 0.000 & 0.000 & 0.701 & 0.964 & 0.935 & 0.953\\
 574 & 0.719 & 0.000 & 0.581 & 0.000 & 0.000 & 0.000 & 0.702 & 0.964 & 0.936 & 0.952\\
 575 & 0.721 & 0.000 & 0.582 & 0.000 & 0.000 & 0.000 & 0.704 & 0.964 & 0.936 & 0.952\\
 576 & 0.724 & 0.000 & 0.586 & 0.000 & 0.000 & 0.000 & 0.707 & 0.965 & 0.937 & 0.952\\
 577 & 0.726 & 0.000 & 0.592 & 0.000 & 0.000 & 0.000 & 0.709 & 0.965 & 0.937 & 0.952\\
 578 & 0.729 & 0.000 & 0.599 & 0.000 & 0.000 & 0.000 & 0.712 & 0.965 & 0.938 & 0.953\\
 579 & 0.732 & 0.000 & 0.606 & 0.000 & 0.000 & 0.000 & 0.715 & 0.965 & 0.938 & 0.954\\
 580 & 0.735 & 0.000 & 0.612 & 0.000 & 0.000 & 0.000 & 0.719 & 0.965 & 0.938 & 0.955\\
 581 & 0.738 & 0.000 & 0.615 & 0.000 & 0.000 & 0.000 & 0.722 & 0.965 & 0.939 & 0.957\\
 582 & 0.741 & 0.000 & 0.617 & 0.000 & 0.000 & 0.000 & 0.725 & 0.965 & 0.939 & 0.958\\
 583 & 0.744 & 0.000 & 0.617 & 0.000 & 0.000 & 0.000 & 0.727 & 0.965 & 0.940 & 0.959\\
 584 & 0.746 & 0.000 & 0.616 & 0.000 & 0.000 & 0.000 & 0.728 & 0.965 & 0.940 & 0.960\\
 585 & 0.748 & 0.000 & 0.614 & 0.000 & 0.000 & 0.000 & 0.729 & 0.965 & 0.940 & 0.961\\
 586 & 0.750 & 0.000 & 0.611 & 0.000 & 0.000 & 0.000 & 0.729 & 0.965 & 0.941 & 0.961\\
 587 & 0.752 & 0.000 & 0.609 & 0.000 & 0.000 & 0.000 & 0.730 & 0.965 & 0.941 & 0.961\\
 588 & 0.754 & 0.000 & 0.609 & 0.000 & 0.000 & 0.000 & 0.731 & 0.966 & 0.942 & 0.960\\
 589 & 0.752 & 0.000 & 0.610 & 0.000 & 0.000 & 0.000 & 0.731 & 0.966 & 0.942 & 0.957\\
 590 & 0.754 & 0.000 & 0.615 & 0.000 & 0.000 & 0.000 & 0.733 & 0.966 & 0.942 & 0.957\\
 591 & 0.758 & 0.000 & 0.621 & 0.000 & 0.000 & 0.000 & 0.738 & 0.966 & 0.943 & 0.958\\
 592 & 0.759 & 0.000 & 0.623 & 0.000 & 0.000 & 0.000 & 0.740 & 0.966 & 0.943 & 0.957\\
 593 & 0.762 & 0.000 & 0.623 & 0.000 & 0.000 & 0.000 & 0.742 & 0.966 & 0.944 & 0.957\\
 594 & 0.764 & 0.000 & 0.621 & 0.000 & 0.000 & 0.000 & 0.742 & 0.966 & 0.944 & 0.957\\
 595 & 0.766 & 0.000 & 0.621 & 0.000 & 0.000 & 0.000 & 0.742 & 0.966 & 0.944 & 0.955\\
 596 & 0.769 & 0.000 & 0.624 & 0.000 & 0.000 & 0.000 & 0.744 & 0.966 & 0.945 & 0.956\\
 597 & 0.770 & 0.000 & 0.628 & 0.000 & 0.000 & 0.000 & 0.743 & 0.966 & 0.945 & 0.956\\
 598 & 0.772 & 0.000 & 0.633 & 0.000 & 0.000 & 0.000 & 0.744 & 0.966 & 0.945 & 0.956\\
 599 & 0.774 & 0.000 & 0.638 & 0.000 & 0.000 & 0.000 & 0.747 & 0.966 & 0.946 & 0.956\\
 600 & 0.776 & 0.000 & 0.641 & 0.000 & 0.000 & 0.000 & 0.751 & 0.966 & 0.946 & 0.956\\
 601 & 0.778 & 0.000 & 0.642 & 0.000 & 0.000 & 0.000 & 0.755 & 0.967 & 0.947 & 0.956\\
 602 & 0.779 & 0.000 & 0.644 & 0.000 & 0.000 & 0.000 & 0.758 & 0.967 & 0.947 & 0.956\\
 603 & 0.781 & 0.000 & 0.647 & 0.000 & 0.000 & 0.000 & 0.761 & 0.967 & 0.947 & 0.956\\
 604 & 0.784 & 0.000 & 0.649 & 0.000 & 0.000 & 0.000 & 0.764 & 0.967 & 0.948 & 0.956\\
 605 & 0.786 & 0.000 & 0.651 & 0.000 & 0.000 & 0.000 & 0.765 & 0.967 & 0.948 & 0.956\\
 606 & 0.788 & 0.000 & 0.652 & 0.000 & 0.000 & 0.000 & 0.766 & 0.967 & 0.948 & 0.957\\
 607 & 0.790 & 0.000 & 0.653 & 0.000 & 0.000 & 0.000 & 0.766 & 0.967 & 0.949 & 0.957\\
 608 & 0.792 & 0.000 & 0.654 & 0.000 & 0.000 & 0.000 & 0.768 & 0.967 & 0.949 & 0.958\\
 609 & 0.795 & 0.000 & 0.655 & 0.000 & 0.000 & 0.000 & 0.771 & 0.967 & 0.949 & 0.959\\
 610 & 0.797 & 0.000 & 0.655 & 0.000 & 0.000 & 0.000 & 0.775 & 0.967 & 0.950 & 0.959\\
 611 & 0.799 & 0.000 & 0.656 & 0.000 & 0.000 & 0.000 & 0.779 & 0.967 & 0.950 & 0.960\\
 612 & 0.801 & 0.000 & 0.656 & 0.000 & 0.000 & 0.000 & 0.782 & 0.967 & 0.950 & 0.961\\
 613 & 0.804 & 0.000 & 0.657 & 0.000 & 0.000 & 0.000 & 0.785 & 0.967 & 0.951 & 0.961\\
 614 & 0.806 & 0.000 & 0.656 & 0.000 & 0.000 & 0.000 & 0.787 & 0.968 & 0.951 & 0.962\\
 615 & 0.807 & 0.000 & 0.653 & 0.000 & 0.000 & 0.000 & 0.788 & 0.968 & 0.951 & 0.962\\
 616 & 0.808 & 0.000 & 0.648 & 0.000 & 0.000 & 0.000 & 0.789 & 0.968 & 0.952 & 0.963\\
 617 & 0.810 & 0.000 & 0.643 & 0.000 & 0.000 & 0.000 & 0.789 & 0.968 & 0.952 & 0.963\\
 618 & 0.812 & 0.000 & 0.640 & 0.000 & 0.000 & 0.000 & 0.791 & 0.968 & 0.952 & 0.964\\
 619 & 0.814 & 0.000 & 0.640 & 0.000 & 0.000 & 0.000 & 0.792 & 0.968 & 0.953 & 0.964\\
 620 & 0.817 & 0.000 & 0.642 & 0.000 & 0.000 & 0.000 & 0.794 & 0.968 & 0.953 & 0.964\\
 621 & 0.820 & 0.000 & 0.645 & 0.000 & 0.000 & 0.000 & 0.797 & 0.968 & 0.953 & 0.964\\
 622 & 0.823 & 0.000 & 0.648 & 0.000 & 0.000 & 0.000 & 0.800 & 0.968 & 0.953 & 0.964\\
 623 & 0.824 & 0.000 & 0.647 & 0.000 & 0.000 & 0.000 & 0.802 & 0.968 & 0.954 & 0.964\\
 624 & 0.825 & 0.000 & 0.646 & 0.000 & 0.000 & 0.000 & 0.804 & 0.968 & 0.954 & 0.964\\
 625 & 0.825 & 0.000 & 0.646 & 0.000 & 0.000 & 0.000 & 0.806 & 0.968 & 0.954 & 0.964\\
 626 & 0.826 & 0.000 & 0.648 & 0.000 & 0.000 & 0.000 & 0.808 & 0.968 & 0.955 & 0.964\\
 627 & 0.828 & 0.000 & 0.652 & 0.000 & 0.000 & 0.000 & 0.810 & 0.968 & 0.955 & 0.964\\
 628 & 0.808 & 0.000 & 0.641 & 0.000 & 0.000 & 0.000 & 0.791 & 0.969 & 0.955 & 0.939\\
 629 & 0.823 & 0.000 & 0.655 & 0.000 & 0.000 & 0.000 & 0.805 & 0.969 & 0.955 & 0.954\\
 630 & 0.823 & 0.000 & 0.657 & 0.000 & 0.000 & 0.000 & 0.804 & 0.969 & 0.956 & 0.953\\
 631 & 0.832 & 0.000 & 0.662 & 0.000 & 0.000 & 0.000 & 0.811 & 0.969 & 0.956 & 0.960\\
 632 & 0.836 & 0.000 & 0.662 & 0.000 & 0.000 & 0.000 & 0.814 & 0.969 & 0.956 & 0.963\\
 633 & 0.840 & 0.000 & 0.660 & 0.000 & 0.000 & 0.000 & 0.817 & 0.969 & 0.957 & 0.966\\
 634 & 0.843 & 0.000 & 0.660 & 0.000 & 0.000 & 0.000 & 0.821 & 0.969 & 0.957 & 0.967\\
 635 & 0.845 & 0.000 & 0.660 & 0.000 & 0.000 & 0.000 & 0.824 & 0.969 & 0.957 & 0.968\\
 636 & 0.847 & 0.000 & 0.663 & 0.000 & 0.000 & 0.000 & 0.828 & 0.969 & 0.957 & 0.970\\
 637 & 0.850 & 0.000 & 0.668 & 0.000 & 0.000 & 0.000 & 0.831 & 0.969 & 0.958 & 0.971\\
 638 & 0.852 & 0.000 & 0.673 & 0.000 & 0.000 & 0.000 & 0.835 & 0.969 & 0.958 & 0.972\\
 639 & 0.855 & 0.000 & 0.678 & 0.000 & 0.000 & 0.000 & 0.838 & 0.969 & 0.958 & 0.973\\
 640 & 0.857 & 0.000 & 0.681 & 0.000 & 0.000 & 0.000 & 0.838 & 0.969 & 0.958 & 0.973\\
 641 & 0.859 & 0.000 & 0.684 & 0.000 & 0.000 & 0.000 & 0.838 & 0.969 & 0.959 & 0.974\\
 642 & 0.860 & 0.000 & 0.685 & 0.000 & 0.000 & 0.000 & 0.836 & 0.969 & 0.959 & 0.975\\
 643 & 0.862 & 0.000 & 0.686 & 0.000 & 0.000 & 0.000 & 0.835 & 0.970 & 0.959 & 0.975\\
 644 & 0.865 & 0.000 & 0.687 & 0.000 & 0.000 & 0.000 & 0.835 & 0.970 & 0.959 & 0.976\\
 645 & 0.866 & 0.000 & 0.686 & 0.000 & 0.000 & 0.000 & 0.835 & 0.970 & 0.960 & 0.976\\
 646 & 0.866 & 0.000 & 0.685 & 0.000 & 0.000 & 0.000 & 0.836 & 0.970 & 0.960 & 0.976\\
 647 & 0.867 & 0.000 & 0.684 & 0.000 & 0.000 & 0.000 & 0.838 & 0.970 & 0.960 & 0.975\\
 648 & 0.867 & 0.000 & 0.683 & 0.000 & 0.000 & 0.000 & 0.842 & 0.970 & 0.960 & 0.973\\
 649 & 0.869 & 0.000 & 0.683 & 0.000 & 0.000 & 0.000 & 0.846 & 0.970 & 0.961 & 0.974\\
 650 & 0.873 & 0.000 & 0.685 & 0.000 & 0.000 & 0.000 & 0.852 & 0.970 & 0.961 & 0.977\\
 651 & 0.875 & 0.000 & 0.686 & 0.000 & 0.000 & 0.000 & 0.856 & 0.970 & 0.961 & 0.978\\
 652 & 0.874 & 0.000 & 0.684 & 0.000 & 0.000 & 0.000 & 0.854 & 0.970 & 0.961 & 0.975\\
 653 & 0.879 & 0.000 & 0.686 & 0.000 & 0.000 & 0.000 & 0.858 & 0.970 & 0.962 & 0.978\\
 654 & 0.881 & 0.000 & 0.687 & 0.000 & 0.000 & 0.000 & 0.858 & 0.970 & 0.962 & 0.979\\
 655 & 0.880 & 0.000 & 0.684 & 0.000 & 0.000 & 0.000 & 0.854 & 0.970 & 0.962 & 0.977\\
 656 & 0.882 & 0.000 & 0.684 & 0.000 & 0.000 & 0.000 & 0.853 & 0.970 & 0.962 & 0.979\\
 657 & 0.883 & 0.000 & 0.682 & 0.000 & 0.000 & 0.000 & 0.852 & 0.970 & 0.963 & 0.980\\
 658 & 0.885 & 0.000 & 0.682 & 0.000 & 0.000 & 0.000 & 0.854 & 0.970 & 0.963 & 0.980\\
 659 & 0.887 & 0.000 & 0.681 & 0.000 & 0.000 & 0.000 & 0.857 & 0.971 & 0.963 & 0.981\\
 660 & 0.889 & 0.000 & 0.679 & 0.000 & 0.000 & 0.000 & 0.861 & 0.971 & 0.963 & 0.982\\
 661 & 0.892 & 0.000 & 0.677 & 0.000 & 0.000 & 0.000 & 0.866 & 0.971 & 0.964 & 0.982\\
 662 & 0.894 & 0.000 & 0.675 & 0.000 & 0.000 & 0.000 & 0.871 & 0.971 & 0.964 & 0.983\\
 663 & 0.895 & 0.000 & 0.672 & 0.000 & 0.000 & 0.000 & 0.875 & 0.971 & 0.964 & 0.983\\
 664 & 0.896 & 0.000 & 0.669 & 0.000 & 0.000 & 0.000 & 0.878 & 0.971 & 0.964 & 0.984\\
 665 & 0.897 & 0.000 & 0.666 & 0.001 & 0.000 & 0.000 & 0.879 & 0.971 & 0.964 & 0.984\\
 666 & 0.898 & 0.000 & 0.664 & 0.001 & 0.000 & 0.000 & 0.878 & 0.971 & 0.965 & 0.984\\
 667 & 0.899 & 0.000 & 0.663 & 0.001 & 0.000 & 0.000 & 0.876 & 0.971 & 0.965 & 0.985\\
 668 & 0.900 & 0.000 & 0.663 & 0.001 & 0.000 & 0.000 & 0.875 & 0.971 & 0.965 & 0.985\\
 669 & 0.902 & 0.000 & 0.663 & 0.001 & 0.000 & 0.000 & 0.873 & 0.971 & 0.965 & 0.985\\
 670 & 0.903 & 0.000 & 0.663 & 0.001 & 0.000 & 0.000 & 0.872 & 0.971 & 0.965 & 0.986\\
 671 & 0.904 & 0.000 & 0.662 & 0.001 & 0.000 & 0.000 & 0.872 & 0.971 & 0.966 & 0.986\\
 672 & 0.906 & 0.000 & 0.662 & 0.002 & 0.000 & 0.000 & 0.873 & 0.971 & 0.966 & 0.986\\
 673 & 0.906 & 0.000 & 0.660 & 0.002 & 0.000 & 0.000 & 0.875 & 0.971 & 0.966 & 0.987\\
 674 & 0.907 & 0.000 & 0.658 & 0.003 & 0.000 & 0.000 & 0.879 & 0.971 & 0.966 & 0.987\\
 675 & 0.908 & 0.000 & 0.655 & 0.004 & 0.000 & 0.000 & 0.883 & 0.971 & 0.966 & 0.987\\
 676 & 0.910 & 0.000 & 0.652 & 0.005 & 0.000 & 0.000 & 0.888 & 0.972 & 0.967 & 0.988\\
 677 & 0.911 & 0.000 & 0.649 & 0.007 & 0.000 & 0.000 & 0.892 & 0.972 & 0.967 & 0.988\\
 678 & 0.912 & 0.000 & 0.644 & 0.009 & 0.000 & 0.000 & 0.896 & 0.972 & 0.967 & 0.988\\
 679 & 0.914 & 0.000 & 0.639 & 0.012 & 0.000 & 0.000 & 0.898 & 0.972 & 0.967 & 0.988\\
 680 & 0.916 & 0.000 & 0.633 & 0.016 & 0.000 & 0.000 & 0.900 & 0.972 & 0.967 & 0.989\\
 681 & 0.917 & 0.000 & 0.626 & 0.022 & 0.000 & 0.000 & 0.899 & 0.972 & 0.968 & 0.989\\
 682 & 0.918 & 0.000 & 0.617 & 0.029 & 0.000 & 0.000 & 0.898 & 0.972 & 0.968 & 0.989\\
 683 & 0.919 & 0.000 & 0.608 & 0.039 & 0.000 & 0.000 & 0.896 & 0.972 & 0.968 & 0.989\\
 684 & 0.920 & 0.000 & 0.595 & 0.056 & 0.000 & 0.000 & 0.895 & 0.972 & 0.968 & 0.989\\
 685 & 0.921 & 0.000 & 0.579 & 0.084 & 0.000 & 0.000 & 0.894 & 0.972 & 0.968 & 0.989\\
 686 & 0.921 & 0.000 & 0.556 & 0.133 & 0.000 & 0.000 & 0.894 & 0.972 & 0.969 & 0.989\\
 687 & 0.750 & 0.000 & 0.427 & 0.169 & 0.000 & 0.000 & 0.728 & 0.972 & 0.969 & 0.805\\
 688 & 0.813 & 0.000 & 0.428 & 0.264 & 0.000 & 0.000 & 0.791 & 0.972 & 0.969 & 0.873\\
 689 & 0.825 & 0.000 & 0.391 & 0.350 & 0.000 & 0.000 & 0.804 & 0.972 & 0.969 & 0.885\\
 690 & 0.835 & 0.000 & 0.346 & 0.426 & 0.000 & 0.000 & 0.817 & 0.972 & 0.969 & 0.895\\
 691 & 0.870 & 0.000 & 0.305 & 0.512 & 0.000 & 0.000 & 0.853 & 0.972 & 0.969 & 0.933\\
 692 & 0.888 & 0.000 & 0.255 & 0.591 & 0.000 & 0.000 & 0.873 & 0.972 & 0.970 & 0.953\\
 693 & 0.901 & 0.000 & 0.204 & 0.670 & 0.000 & 0.000 & 0.888 & 0.973 & 0.970 & 0.967\\
 694 & 0.908 & 0.000 & 0.156 & 0.737 & 0.000 & 0.000 & 0.895 & 0.973 & 0.970 & 0.974\\
 695 & 0.917 & 0.000 & 0.116 & 0.792 & 0.000 & 0.000 & 0.903 & 0.973 & 0.970 & 0.982\\
 696 & 0.918 & 0.000 & 0.084 & 0.821 & 0.000 & 0.000 & 0.903 & 0.973 & 0.970 & 0.981\\
 697 & 0.929 & 0.000 & 0.060 & 0.843 & 0.000 & 0.000 & 0.912 & 0.973 & 0.970 & 0.990\\
 698 & 0.930 & 0.000 & 0.042 & 0.848 & 0.000 & 0.000 & 0.911 & 0.973 & 0.971 & 0.990\\
 699 & 0.926 & 0.000 & 0.029 & 0.846 & 0.000 & 0.000 & 0.905 & 0.973 & 0.971 & 0.986\\
 700 & 0.926 & 0.000 & 0.021 & 0.848 & 0.000 & 0.000 & 0.904 & 0.973 & 0.971 & 0.986\\
 701 & 0.925 & 0.000 & 0.015 & 0.847 & 0.000 & 0.000 & 0.902 & 0.973 & 0.971 & 0.986\\
 702 & 0.926 & 0.000 & 0.011 & 0.847 & 0.000 & 0.000 & 0.903 & 0.973 & 0.971 & 0.987\\
 703 & 0.926 & 0.000 & 0.008 & 0.845 & 0.000 & 0.000 & 0.904 & 0.973 & 0.971 & 0.987\\
 704 & 0.930 & 0.000 & 0.006 & 0.848 & 0.000 & 0.000 & 0.908 & 0.973 & 0.972 & 0.989\\
 705 & 0.931 & 0.000 & 0.005 & 0.849 & 0.000 & 0.000 & 0.911 & 0.973 & 0.972 & 0.989\\
 706 & 0.934 & 0.000 & 0.004 & 0.852 & 0.000 & 0.000 & 0.914 & 0.973 & 0.972 & 0.991\\
 707 & 0.935 & 0.000 & 0.003 & 0.853 & 0.000 & 0.000 & 0.916 & 0.973 & 0.972 & 0.991\\
 708 & 0.936 & 0.000 & 0.002 & 0.851 & 0.000 & 0.000 & 0.917 & 0.973 & 0.972 & 0.991\\
 709 & 0.937 & 0.000 & 0.002 & 0.849 & 0.000 & 0.000 & 0.919 & 0.974 & 0.972 & 0.992\\
 710 & 0.937 & 0.000 & 0.001 & 0.847 & 0.000 & 0.000 & 0.918 & 0.974 & 0.973 & 0.992\\
 711 & 0.938 & 0.000 & 0.001 & 0.847 & 0.000 & 0.000 & 0.917 & 0.974 & 0.973 & 0.992\\
 712 & 0.939 & 0.000 & 0.001 & 0.849 & 0.000 & 0.000 & 0.916 & 0.974 & 0.973 & 0.993\\
 713 & 0.938 & 0.000 & 0.001 & 0.852 & 0.000 & 0.000 & 0.914 & 0.974 & 0.973 & 0.993\\
 714 & 0.938 & 0.000 & 0.000 & 0.855 & 0.000 & 0.000 & 0.912 & 0.974 & 0.973 & 0.992\\
 715 & 0.936 & 0.000 & 0.000 & 0.857 & 0.000 & 0.000 & 0.910 & 0.974 & 0.973 & 0.991\\
 716 & 0.935 & 0.000 & 0.000 & 0.859 & 0.000 & 0.000 & 0.908 & 0.974 & 0.974 & 0.991\\
 717 & 0.917 & 0.000 & 0.000 & 0.844 & 0.000 & 0.000 & 0.891 & 0.974 & 0.974 & 0.972\\
 718 & 0.904 & 0.000 & 0.000 & 0.833 & 0.000 & 0.000 & 0.879 & 0.974 & 0.974 & 0.958\\
 719 & 0.885 & 0.000 & 0.000 & 0.816 & 0.000 & 0.000 & 0.862 & 0.974 & 0.974 & 0.938\\
 720 & 0.894 & 0.000 & 0.000 & 0.825 & 0.000 & 0.000 & 0.872 & 0.974 & 0.974 & 0.946\\
 721 & 0.912 & 0.000 & 0.000 & 0.842 & 0.000 & 0.000 & 0.890 & 0.974 & 0.974 & 0.963\\
 722 & 0.936 & 0.000 & 0.000 & 0.863 & 0.000 & 0.000 & 0.914 & 0.974 & 0.974 & 0.988\\
 723 & 0.920 & 0.000 & 0.000 & 0.846 & 0.000 & 0.000 & 0.898 & 0.974 & 0.975 & 0.971\\
 724 & 0.906 & 0.000 & 0.000 & 0.833 & 0.000 & 0.000 & 0.886 & 0.974 & 0.975 & 0.959\\
 725 & 0.907 & 0.000 & 0.000 & 0.833 & 0.000 & 0.000 & 0.885 & 0.975 & 0.975 & 0.959\\
 726 & 0.917 & 0.000 & 0.000 & 0.842 & 0.000 & 0.000 & 0.894 & 0.975 & 0.975 & 0.970\\
 727 & 0.910 & 0.000 & 0.000 & 0.835 & 0.000 & 0.000 & 0.887 & 0.975 & 0.975 & 0.965\\
 728 & 0.911 & 0.000 & 0.000 & 0.833 & 0.000 & 0.000 & 0.887 & 0.975 & 0.975 & 0.966\\
 729 & 0.914 & 0.000 & 0.000 & 0.831 & 0.000 & 0.000 & 0.888 & 0.975 & 0.975 & 0.969\\
 730 & 0.925 & 0.000 & 0.000 & 0.838 & 0.000 & 0.000 & 0.899 & 0.975 & 0.975 & 0.981\\
 731 & 0.916 & 0.000 & 0.000 & 0.828 & 0.000 & 0.000 & 0.889 & 0.975 & 0.976 & 0.970\\
 732 & 0.927 & 0.000 & 0.000 & 0.838 & 0.000 & 0.000 & 0.900 & 0.975 & 0.976 & 0.982\\
 733 & 0.935 & 0.000 & 0.000 & 0.846 & 0.000 & 0.000 & 0.908 & 0.975 & 0.976 & 0.989\\
 734 & 0.937 & 0.000 & 0.000 & 0.850 & 0.000 & 0.000 & 0.910 & 0.975 & 0.976 & 0.990\\
 735 & 0.938 & 0.000 & 0.000 & 0.853 & 0.000 & 0.000 & 0.912 & 0.975 & 0.976 & 0.990\\
 736 & 0.939 & 0.000 & 0.000 & 0.857 & 0.000 & 0.000 & 0.915 & 0.975 & 0.976 & 0.991\\
 737 & 0.940 & 0.000 & 0.000 & 0.860 & 0.000 & 0.000 & 0.916 & 0.975 & 0.976 & 0.990\\
 738 & 0.944 & 0.000 & 0.000 & 0.864 & 0.000 & 0.000 & 0.921 & 0.975 & 0.977 & 0.994\\
 739 & 0.943 & 0.000 & 0.000 & 0.864 & 0.000 & 0.000 & 0.920 & 0.975 & 0.977 & 0.993\\
 740 & 0.944 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.922 & 0.975 & 0.977 & 0.995\\
 741 & 0.944 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.922 & 0.975 & 0.977 & 0.995\\
 742 & 0.945 & 0.000 & 0.000 & 0.866 & 0.000 & 0.000 & 0.922 & 0.976 & 0.977 & 0.996\\
 743 & 0.944 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.921 & 0.976 & 0.977 & 0.996\\
 744 & 0.944 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.920 & 0.976 & 0.977 & 0.996\\
 745 & 0.944 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.920 & 0.976 & 0.977 & 0.996\\
 746 & 0.945 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.920 & 0.976 & 0.978 & 0.996\\
 747 & 0.945 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.920 & 0.976 & 0.978 & 0.996\\
 748 & 0.946 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.921 & 0.976 & 0.978 & 0.996\\
 749 & 0.947 & 0.000 & 0.000 & 0.867 & 0.000 & 0.000 & 0.922 & 0.976 & 0.978 & 0.996\\
 750 & 0.948 & 0.000 & 0.000 & 0.868 & 0.000 & 0.000 & 0.923 & 0.976 & 0.978 & 0.997\\
 751 & 0.948 & 0.000 & 0.000 & 0.868 & 0.000 & 0.000 & 0.924 & 0.976 & 0.978 & 0.997\\
 752 & 0.949 & 0.000 & 0.000 & 0.869 & 0.000 & 0.000 & 0.924 & 0.976 & 0.978 & 0.997\\
 753 & 0.949 & 0.000 & 0.000 & 0.868 & 0.000 & 0.000 & 0.925 & 0.976 & 0.978 & 0.997\\
 754 & 0.948 & 0.000 & 0.000 & 0.868 & 0.000 & 0.000 & 0.925 & 0.976 & 0.978 & 0.997\\
 755 & 0.948 & 0.000 & 0.000 & 0.867 & 0.000 & 0.000 & 0.925 & 0.976 & 0.979 & 0.997\\
 756 & 0.948 & 0.000 & 0.000 & 0.866 & 0.000 & 0.000 & 0.926 & 0.976 & 0.979 & 0.998\\
 757 & 0.947 & 0.000 & 0.000 & 0.864 & 0.000 & 0.000 & 0.925 & 0.976 & 0.979 & 0.998\\
 758 & 0.946 & 0.000 & 0.000 & 0.863 & 0.000 & 0.000 & 0.925 & 0.976 & 0.979 & 0.998\\
 759 & 0.943 & 0.000 & 0.000 & 0.860 & 0.000 & 0.000 & 0.923 & 0.976 & 0.979 & 0.995\\
 760 & 0.448 & 0.000 & 0.000 & 0.408 & 0.000 & 0.000 & 0.438 & 0.977 & 0.979 & 0.472\\
 761 & 0.364 & 0.000 & 0.000 & 0.331 & 0.000 & 0.000 & 0.356 & 0.977 & 0.979 & 0.383\\
 762 & 0.719 & 0.000 & 0.000 & 0.655 & 0.000 & 0.000 & 0.703 & 0.977 & 0.979 & 0.757\\
 763 & 0.501 & 0.000 & 0.000 & 0.456 & 0.000 & 0.000 & 0.489 & 0.977 & 0.979 & 0.528\\
 764 & 0.617 & 0.000 & 0.000 & 0.562 & 0.000 & 0.000 & 0.602 & 0.977 & 0.980 & 0.650\\
 765 & 0.702 & 0.000 & 0.000 & 0.640 & 0.000 & 0.000 & 0.684 & 0.977 & 0.980 & 0.741\\
 766 & 0.800 & 0.000 & 0.000 & 0.730 & 0.000 & 0.000 & 0.778 & 0.977 & 0.980 & 0.844\\
 767 & 0.857 & 0.000 & 0.000 & 0.783 & 0.000 & 0.000 & 0.832 & 0.977 & 0.980 & 0.905\\
 768 & 0.911 & 0.000 & 0.000 & 0.833 & 0.000 & 0.000 & 0.883 & 0.977 & 0.980 & 0.962\\
 769 & 0.923 & 0.000 & 0.000 & 0.845 & 0.000 & 0.000 & 0.893 & 0.977 & 0.980 & 0.975\\
 770 & 0.938 & 0.000 & 0.000 & 0.859 & 0.000 & 0.000 & 0.906 & 0.977 & 0.980 & 0.989\\
 771 & 0.943 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.910 & 0.977 & 0.980 & 0.995\\
 772 & 0.944 & 0.000 & 0.000 & 0.865 & 0.000 & 0.000 & 0.910 & 0.977 & 0.980 & 0.996\\
 773 & 0.943 & 0.000 & 0.000 & 0.863 & 0.000 & 0.000 & 0.909 & 0.977 & 0.980 & 0.997\\
 774 & 0.942 & 0.000 & 0.000 & 0.860 & 0.000 & 0.000 & 0.910 & 0.977 & 0.981 & 0.997\\
 775 & 0.942 & 0.000 & 0.000 & 0.858 & 0.000 & 0.000 & 0.911 & 0.977 & 0.981 & 0.997\\
 776 & 0.943 & 0.000 & 0.000 & 0.855 & 0.000 & 0.000 & 0.913 & 0.977 & 0.981 & 0.997\\
 777 & 0.943 & 0.000 & 0.000 & 0.853 & 0.000 & 0.000 & 0.915 & 0.977 & 0.981 & 0.997\\
 778 & 0.943 & 0.000 & 0.000 & 0.851 & 0.000 & 0.000 & 0.917 & 0.977 & 0.981 & 0.997\\
 779 & 0.943 & 0.000 & 0.000 & 0.848 & 0.000 & 0.000 & 0.918 & 0.978 & 0.981 & 0.997\\
 780 & 0.943 & 0.000 & 0.000 & 0.844 & 0.000 & 0.000 & 0.919 & 0.978 & 0.981 & 0.997\\
 781 & 0.942 & 0.000 & 0.000 & 0.842 & 0.000 & 0.000 & 0.919 & 0.978 & 0.981 & 0.997\\
 782 & 0.942 & 0.000 & 0.000 & 0.841 & 0.000 & 0.000 & 0.918 & 0.978 & 0.981 & 0.998\\
 783 & 0.942 & 0.000 & 0.000 & 0.840 & 0.000 & 0.000 & 0.917 & 0.978 & 0.982 & 0.998\\
 784 & 0.941 & 0.000 & 0.000 & 0.838 & 0.000 & 0.000 & 0.915 & 0.978 & 0.982 & 0.998\\
 785 & 0.940 & 0.000 & 0.000 & 0.836 & 0.001 & 0.000 & 0.913 & 0.978 & 0.982 & 0.998\\
 786 & 0.939 & 0.000 & 0.000 & 0.833 & 0.001 & 0.000 & 0.911 & 0.978 & 0.982 & 0.997\\
 787 & 0.937 & 0.000 & 0.000 & 0.830 & 0.001 & 0.000 & 0.908 & 0.978 & 0.982 & 0.996\\
 788 & 0.937 & 0.000 & 0.000 & 0.828 & 0.001 & 0.000 & 0.906 & 0.978 & 0.982 & 0.996\\
 789 & 0.936 & 0.000 & 0.000 & 0.824 & 0.001 & 0.000 & 0.905 & 0.978 & 0.982 & 0.995\\
 790 & 0.933 & 0.000 & 0.000 & 0.820 & 0.001 & 0.000 & 0.904 & 0.978 & 0.982 & 0.992\\
 791 & 0.934 & 0.000 & 0.000 & 0.822 & 0.001 & 0.000 & 0.907 & 0.978 & 0.982 & 0.995\\
 792 & 0.934 & 0.000 & 0.000 & 0.824 & 0.001 & 0.000 & 0.908 & 0.978 & 0.982 & 0.995\\
 793 & 0.933 & 0.000 & 0.000 & 0.827 & 0.001 & 0.000 & 0.909 & 0.978 & 0.982 & 0.995\\
 794 & 0.936 & 0.000 & 0.000 & 0.834 & 0.002 & 0.000 & 0.913 & 0.978 & 0.982 & 0.998\\
 795 & 0.937 & 0.000 & 0.000 & 0.838 & 0.002 & 0.000 & 0.915 & 0.978 & 0.983 & 0.997\\
 796 & 0.933 & 0.000 & 0.000 & 0.838 & 0.002 & 0.000 & 0.912 & 0.978 & 0.983 & 0.993\\
 797 & 0.935 & 0.000 & 0.000 & 0.843 & 0.003 & 0.000 & 0.914 & 0.978 & 0.983 & 0.994\\
 798 & 0.938 & 0.000 & 0.000 & 0.846 & 0.004 & 0.000 & 0.916 & 0.978 & 0.983 & 0.997\\
 799 & 0.936 & 0.000 & 0.000 & 0.844 & 0.005 & 0.000 & 0.914 & 0.978 & 0.983 & 0.996\\
 800 & 0.933 & 0.000 & 0.000 & 0.841 & 0.006 & 0.000 & 0.911 & 0.979 & 0.983 & 0.995\\
 801 & 0.931 & 0.000 & 0.000 & 0.838 & 0.007 & 0.000 & 0.907 & 0.979 & 0.983 & 0.995\\
 802 & 0.930 & 0.000 & 0.000 & 0.835 & 0.008 & 0.000 & 0.903 & 0.979 & 0.983 & 0.994\\
 803 & 0.930 & 0.000 & 0.000 & 0.834 & 0.009 & 0.000 & 0.900 & 0.979 & 0.983 & 0.994\\
 804 & 0.932 & 0.000 & 0.000 & 0.832 & 0.012 & 0.000 & 0.895 & 0.979 & 0.983 & 0.995\\
 805 & 0.933 & 0.000 & 0.000 & 0.830 & 0.015 & 0.000 & 0.884 & 0.979 & 0.983 & 0.996\\
 806 & 0.935 & 0.000 & 0.000 & 0.828 & 0.019 & 0.000 & 0.868 & 0.979 & 0.983 & 0.997\\
 807 & 0.934 & 0.000 & 0.000 & 0.824 & 0.025 & 0.000 & 0.840 & 0.979 & 0.984 & 0.997\\
 808 & 0.934 & 0.000 & 0.000 & 0.821 & 0.034 & 0.000 & 0.804 & 0.979 & 0.984 & 0.997\\
 809 & 0.932 & 0.000 & 0.000 & 0.817 & 0.045 & 0.000 & 0.758 & 0.979 & 0.984 & 0.996\\
 810 & 0.930 & 0.000 & 0.000 & 0.813 & 0.060 & 0.000 & 0.704 & 0.979 & 0.984 & 0.994\\
 811 & 0.930 & 0.000 & 0.000 & 0.810 & 0.079 & 0.000 & 0.644 & 0.979 & 0.984 & 0.994\\
 812 & 0.925 & 0.000 & 0.000 & 0.804 & 0.101 & 0.000 & 0.578 & 0.979 & 0.984 & 0.990\\
 813 & 0.920 & 0.000 & 0.000 & 0.798 & 0.129 & 0.000 & 0.512 & 0.979 & 0.984 & 0.986\\
 814 & 0.904 & 0.000 & 0.000 & 0.780 & 0.160 & 0.000 & 0.442 & 0.979 & 0.984 & 0.969\\
 815 & 0.902 & 0.000 & 0.000 & 0.767 & 0.203 & 0.000 & 0.384 & 0.979 & 0.984 & 0.968\\
 816 & 0.885 & 0.000 & 0.000 & 0.728 & 0.252 & 0.000 & 0.325 & 0.979 & 0.984 & 0.949\\
 817 & 0.887 & 0.000 & 0.000 & 0.684 & 0.318 & 0.000 & 0.280 & 0.979 & 0.984 & 0.953\\
 818 & 0.883 & 0.000 & 0.000 & 0.609 & 0.397 & 0.000 & 0.238 & 0.979 & 0.984 & 0.950\\
 819 & 0.902 & 0.000 & 0.000 & 0.523 & 0.499 & 0.000 & 0.206 & 0.979 & 0.985 & 0.970\\
 820 & 0.892 & 0.000 & 0.000 & 0.408 & 0.588 & 0.000 & 0.172 & 0.979 & 0.985 & 0.959\\
 821 & 0.921 & 0.000 & 0.000 & 0.313 & 0.696 & 0.000 & 0.149 & 0.979 & 0.985 & 0.990\\
 822 & 0.916 & 0.000 & 0.000 & 0.221 & 0.761 & 0.000 & 0.123 & 0.979 & 0.985 & 0.984\\
 823 & 0.851 & 0.000 & 0.000 & 0.142 & 0.750 & 0.000 & 0.094 & 0.980 & 0.985 & 0.914\\
 824 & 0.913 & 0.000 & 0.000 & 0.104 & 0.833 & 0.000 & 0.082 & 0.980 & 0.985 & 0.982\\
 825 & 0.914 & 0.000 & 0.000 & 0.071 & 0.849 & 0.000 & 0.066 & 0.980 & 0.985 & 0.984\\
 826 & 0.907 & 0.000 & 0.000 & 0.047 & 0.850 & 0.000 & 0.053 & 0.980 & 0.985 & 0.978\\
 827 & 0.916 & 0.000 & 0.000 & 0.033 & 0.863 & 0.000 & 0.042 & 0.980 & 0.985 & 0.988\\
 828 & 0.887 & 0.000 & 0.000 & 0.021 & 0.839 & 0.000 & 0.033 & 0.980 & 0.985 & 0.957\\
 829 & 0.906 & 0.000 & 0.000 & 0.015 & 0.860 & 0.000 & 0.027 & 0.980 & 0.985 & 0.979\\
 830 & 0.904 & 0.000 & 0.000 & 0.010 & 0.858 & 0.000 & 0.021 & 0.980 & 0.985 & 0.978\\
 831 & 0.904 & 0.000 & 0.000 & 0.007 & 0.857 & 0.000 & 0.017 & 0.980 & 0.985 & 0.979\\
 832 & 0.895 & 0.000 & 0.000 & 0.005 & 0.845 & 0.000 & 0.014 & 0.980 & 0.985 & 0.970\\
 833 & 0.915 & 0.000 & 0.000 & 0.004 & 0.862 & 0.000 & 0.012 & 0.980 & 0.986 & 0.991\\
 834 & 0.909 & 0.000 & 0.000 & 0.003 & 0.857 & 0.000 & 0.010 & 0.980 & 0.986 & 0.986\\
 835 & 0.919 & 0.000 & 0.000 & 0.002 & 0.867 & 0.000 & 0.008 & 0.980 & 0.986 & 0.996\\
 836 & 0.915 & 0.000 & 0.000 & 0.002 & 0.867 & 0.000 & 0.007 & 0.980 & 0.986 & 0.990\\
 837 & 0.921 & 0.000 & 0.000 & 0.001 & 0.877 & 0.000 & 0.006 & 0.980 & 0.986 & 0.996\\
 838 & 0.920 & 0.000 & 0.000 & 0.001 & 0.879 & 0.000 & 0.006 & 0.980 & 0.986 & 0.995\\
 839 & 0.920 & 0.000 & 0.000 & 0.001 & 0.880 & 0.000 & 0.005 & 0.980 & 0.986 & 0.997\\
 840 & 0.920 & 0.000 & 0.000 & 0.001 & 0.880 & 0.000 & 0.004 & 0.980 & 0.986 & 0.997\\
 841 & 0.918 & 0.000 & 0.000 & 0.001 & 0.876 & 0.000 & 0.004 & 0.980 & 0.986 & 0.996\\
 842 & 0.917 & 0.000 & 0.000 & 0.001 & 0.873 & 0.000 & 0.004 & 0.980 & 0.986 & 0.997\\
 843 & 0.917 & 0.000 & 0.000 & 0.001 & 0.871 & 0.000 & 0.004 & 0.980 & 0.986 & 0.998\\
 844 & 0.915 & 0.000 & 0.000 & 0.000 & 0.869 & 0.000 & 0.003 & 0.980 & 0.986 & 0.997\\
 845 & 0.915 & 0.000 & 0.000 & 0.000 & 0.869 & 0.000 & 0.003 & 0.980 & 0.986 & 0.999\\
 846 & 0.914 & 0.000 & 0.000 & 0.000 & 0.868 & 0.000 & 0.003 & 0.980 & 0.986 & 0.998\\
 847 & 0.913 & 0.000 & 0.000 & 0.000 & 0.868 & 0.000 & 0.003 & 0.981 & 0.986 & 0.999\\
 848 & 0.911 & 0.000 & 0.000 & 0.000 & 0.867 & 0.000 & 0.002 & 0.981 & 0.987 & 0.998\\
 849 & 0.911 & 0.000 & 0.000 & 0.000 & 0.866 & 0.000 & 0.002 & 0.981 & 0.987 & 0.998\\
 850 & 0.910 & 0.000 & 0.000 & 0.000 & 0.865 & 0.000 & 0.002 & 0.981 & 0.987 & 0.998\\
 851 & 0.909 & 0.000 & 0.000 & 0.000 & 0.863 & 0.000 & 0.002 & 0.981 & 0.987 & 0.997\\
 852 & 0.909 & 0.000 & 0.000 & 0.000 & 0.861 & 0.000 & 0.001 & 0.981 & 0.987 & 0.998\\
 853 & 0.909 & 0.000 & 0.000 & 0.000 & 0.858 & 0.000 & 0.001 & 0.981 & 0.987 & 0.998\\
 854 & 0.908 & 0.000 & 0.000 & 0.000 & 0.855 & 0.000 & 0.001 & 0.981 & 0.987 & 0.998\\
 855 & 0.907 & 0.000 & 0.000 & 0.000 & 0.854 & 0.000 & 0.001 & 0.981 & 0.987 & 0.999\\
 856 & 0.906 & 0.000 & 0.000 & 0.000 & 0.852 & 0.000 & 0.001 & 0.981 & 0.987 & 0.998\\
 857 & 0.904 & 0.000 & 0.000 & 0.000 & 0.850 & 0.000 & 0.001 & 0.981 & 0.987 & 0.999\\
 858 & 0.902 & 0.000 & 0.000 & 0.000 & 0.848 & 0.000 & 0.001 & 0.981 & 0.987 & 0.999\\
 859 & 0.901 & 0.000 & 0.000 & 0.000 & 0.848 & 0.000 & 0.001 & 0.981 & 0.987 & 0.999\\
 860 & 0.900 & 0.000 & 0.000 & 0.000 & 0.849 & 0.000 & 0.000 & 0.981 & 0.987 & 0.999\\
 861 & 0.900 & 0.000 & 0.000 & 0.000 & 0.850 & 0.000 & 0.000 & 0.981 & 0.987 & 0.999\\
 862 & 0.899 & 0.000 & 0.000 & 0.000 & 0.851 & 0.000 & 0.000 & 0.981 & 0.987 & 0.999\\
 863 & 0.898 & 0.000 & 0.000 & 0.000 & 0.850 & 0.000 & 0.000 & 0.981 & 0.987 & 0.999\\
 864 & 0.897 & 0.000 & 0.000 & 0.000 & 0.849 & 0.000 & 0.000 & 0.981 & 0.988 & 0.999\\
 865 & 0.896 & 0.000 & 0.000 & 0.000 & 0.849 & 0.000 & 0.000 & 0.981 & 0.988 & 0.999\\
 866 & 0.896 & 0.000 & 0.000 & 0.000 & 0.848 & 0.000 & 0.000 & 0.981 & 0.988 & 0.999\\
 867 & 0.895 & 0.000 & 0.000 & 0.000 & 0.846 & 0.000 & 0.000 & 0.981 & 0.988 & 0.999\\
 868 & 0.893 & 0.000 & 0.000 & 0.000 & 0.845 & 0.000 & 0.000 & 0.981 & 0.988 & 1.000\\
 869 & 0.892 & 0.000 & 0.000 & 0.000 & 0.843 & 0.000 & 0.000 & 0.981 & 0.988 & 1.000\\
 870 & 0.891 & 0.000 & 0.000 & 0.000 & 0.840 & 0.000 & 0.000 & 0.981 & 0.988 & 1.000\\
 871 & 0.889 & 0.000 & 0.000 & 0.000 & 0.839 & 0.000 & 0.000 & 0.981 & 0.988 & 1.000\\
 872 & 0.887 & 0.000 & 0.000 & 0.000 & 0.837 & 0.000 & 0.000 & 0.981 & 0.988 & 1.000\\
 873 & 0.885 & 0.000 & 0.000 & 0.000 & 0.835 & 0.000 & 0.000 & 0.981 & 0.988 & 1.000\\
 874 & 0.883 & 0.000 & 0.000 & 0.000 & 0.833 & 0.000 & 0.000 & 0.982 & 0.988 & 1.000\\
 875 & 0.881 & 0.000 & 0.000 & 0.000 & 0.832 & 0.000 & 0.000 & 0.982 & 0.988 & 1.000\\
 876 & 0.878 & 0.000 & 0.000 & 0.000 & 0.831 & 0.000 & 0.000 & 0.982 & 0.988 & 1.000\\
 877 & 0.877 & 0.000 & 0.000 & 0.000 & 0.829 & 0.000 & 0.000 & 0.982 & 0.988 & 1.000\\
 878 & 0.874 & 0.000 & 0.000 & 0.000 & 0.827 & 0.000 & 0.000 & 0.982 & 0.988 & 1.000\\
 879 & 0.872 & 0.000 & 0.000 & 0.000 & 0.824 & 0.000 & 0.000 & 0.982 & 0.988 & 1.000\\
 880 & 0.869 & 0.000 & 0.000 & 0.000 & 0.820 & 0.000 & 0.000 & 0.982 & 0.988 & 1.000\\
 881 & 0.866 & 0.000 & 0.000 & 0.000 & 0.816 & 0.000 & 0.000 & 0.982 & 0.988 & 0.999\\
 882 & 0.863 & 0.000 & 0.000 & 0.000 & 0.810 & 0.000 & 0.000 & 0.982 & 0.989 & 0.999\\
 883 & 0.861 & 0.000 & 0.000 & 0.000 & 0.806 & 0.000 & 0.000 & 0.982 & 0.989 & 0.999\\
 884 & 0.859 & 0.000 & 0.000 & 0.000 & 0.801 & 0.000 & 0.000 & 0.982 & 0.989 & 0.999\\
 885 & 0.857 & 0.000 & 0.000 & 0.000 & 0.796 & 0.000 & 0.000 & 0.982 & 0.989 & 0.999\\
 886 & 0.854 & 0.000 & 0.000 & 0.000 & 0.792 & 0.000 & 0.000 & 0.982 & 0.989 & 0.998\\
 887 & 0.851 & 0.000 & 0.000 & 0.000 & 0.790 & 0.000 & 0.000 & 0.982 & 0.989 & 0.999\\
 888 & 0.846 & 0.000 & 0.000 & 0.000 & 0.787 & 0.000 & 0.000 & 0.982 & 0.989 & 0.998\\
 889 & 0.844 & 0.000 & 0.000 & 0.000 & 0.786 & 0.000 & 0.000 & 0.982 & 0.989 & 1.000\\
 890 & 0.839 & 0.000 & 0.000 & 0.000 & 0.783 & 0.000 & 0.000 & 0.982 & 0.989 & 0.998\\
 891 & 0.838 & 0.000 & 0.000 & 0.000 & 0.783 & 0.000 & 0.000 & 0.982 & 0.989 & 0.999\\
 892 & 0.836 & 0.000 & 0.000 & 0.000 & 0.781 & 0.000 & 0.000 & 0.982 & 0.989 & 0.997\\
 893 & 0.830 & 0.000 & 0.000 & 0.000 & 0.777 & 0.000 & 0.000 & 0.982 & 0.989 & 0.993\\
 894 & 0.825 & 0.000 & 0.000 & 0.000 & 0.773 & 0.000 & 0.000 & 0.982 & 0.989 & 0.990\\
 895 & 0.817 & 0.000 & 0.000 & 0.000 & 0.764 & 0.000 & 0.000 & 0.982 & 0.989 & 0.984\\
 896 & 0.801 & 0.000 & 0.000 & 0.000 & 0.747 & 0.000 & 0.000 & 0.982 & 0.989 & 0.968\\
 897 & 0.778 & 0.000 & 0.000 & 0.000 & 0.723 & 0.001 & 0.000 & 0.982 & 0.989 & 0.943\\
 898 & 0.786 & 0.000 & 0.000 & 0.000 & 0.727 & 0.001 & 0.000 & 0.982 & 0.989 & 0.956\\
 899 & 0.729 & 0.000 & 0.000 & 0.000 & 0.671 & 0.001 & 0.000 & 0.982 & 0.989 & 0.890\\
 900 & 0.783 & 0.000 & 0.000 & 0.000 & 0.719 & 0.001 & 0.000 & 0.982 & 0.989 & 0.960\\
 901 & 0.760 & 0.000 & 0.000 & 0.000 & 0.697 & 0.002 & 0.000 & 0.982 & 0.989 & 0.934\\
 902 & 0.773 & 0.000 & 0.000 & 0.000 & 0.710 & 0.002 & 0.000 & 0.983 & 0.990 & 0.955\\
 903 & 0.752 & 0.000 & 0.000 & 0.000 & 0.691 & 0.002 & 0.000 & 0.983 & 0.990 & 0.934\\
 904 & 0.793 & 0.000 & 0.000 & 0.000 & 0.730 & 0.002 & 0.000 & 0.983 & 0.990 & 0.990\\
 905 & 0.785 & 0.000 & 0.000 & 0.000 & 0.725 & 0.002 & 0.000 & 0.983 & 0.990 & 0.985\\
 906 & 0.770 & 0.000 & 0.000 & 0.000 & 0.714 & 0.003 & 0.000 & 0.983 & 0.990 & 0.972\\
 907 & 0.738 & 0.000 & 0.000 & 0.000 & 0.687 & 0.003 & 0.000 & 0.983 & 0.990 & 0.936\\
 908 & 0.738 & 0.000 & 0.000 & 0.000 & 0.688 & 0.003 & 0.000 & 0.983 & 0.990 & 0.940\\
 909 & 0.744 & 0.000 & 0.000 & 0.000 & 0.694 & 0.005 & 0.000 & 0.983 & 0.990 & 0.952\\
 910 & 0.731 & 0.000 & 0.000 & 0.000 & 0.683 & 0.006 & 0.000 & 0.983 & 0.990 & 0.941\\
 911 & 0.740 & 0.000 & 0.000 & 0.000 & 0.691 & 0.009 & 0.000 & 0.983 & 0.990 & 0.959\\
 912 & 0.731 & 0.000 & 0.000 & 0.000 & 0.680 & 0.015 & 0.000 & 0.983 & 0.990 & 0.952\\
 913 & 0.720 & 0.000 & 0.000 & 0.000 & 0.666 & 0.024 & 0.000 & 0.983 & 0.990 & 0.943\\
 914 & 0.711 & 0.000 & 0.000 & 0.000 & 0.653 & 0.040 & 0.000 & 0.983 & 0.990 & 0.937\\
 915 & 0.723 & 0.000 & 0.000 & 0.000 & 0.659 & 0.066 & 0.000 & 0.983 & 0.990 & 0.960\\
 916 & 0.694 & 0.000 & 0.000 & 0.000 & 0.625 & 0.098 & 0.000 & 0.983 & 0.990 & 0.927\\
 917 & 0.725 & 0.000 & 0.000 & 0.000 & 0.642 & 0.152 & 0.000 & 0.983 & 0.990 & 0.975\\
 918 & 0.686 & 0.000 & 0.000 & 0.000 & 0.592 & 0.199 & 0.000 & 0.983 & 0.990 & 0.930\\
 919 & 0.711 & 0.000 & 0.000 & 0.000 & 0.590 & 0.271 & 0.000 & 0.983 & 0.990 & 0.971\\
 920 & 0.705 & 0.000 & 0.000 & 0.000 & 0.549 & 0.335 & 0.000 & 0.983 & 0.990 & 0.970\\
 921 & 0.711 & 0.000 & 0.000 & 0.000 & 0.504 & 0.403 & 0.000 & 0.983 & 0.990 & 0.986\\
 922 & 0.693 & 0.000 & 0.000 & 0.000 & 0.429 & 0.451 & 0.000 & 0.983 & 0.990 & 0.969\\
 923 & 0.699 & 0.000 & 0.000 & 0.000 & 0.361 & 0.506 & 0.000 & 0.983 & 0.990 & 0.984\\
 924 & 0.687 & 0.000 & 0.000 & 0.000 & 0.283 & 0.539 & 0.000 & 0.983 & 0.990 & 0.976\\
 925 & 0.677 & 0.000 & 0.000 & 0.000 & 0.214 & 0.565 & 0.000 & 0.983 & 0.990 & 0.970\\
 926 & 0.675 & 0.000 & 0.000 & 0.000 & 0.158 & 0.591 & 0.000 & 0.983 & 0.991 & 0.976\\
 927 & 0.679 & 0.000 & 0.000 & 0.000 & 0.116 & 0.615 & 0.000 & 0.983 & 0.991 & 0.988\\
 928 & 0.642 & 0.000 & 0.000 & 0.000 & 0.079 & 0.597 & 0.000 & 0.983 & 0.991 & 0.943\\
 929 & 0.635 & 0.000 & 0.000 & 0.000 & 0.057 & 0.601 & 0.000 & 0.983 & 0.991 & 0.941\\
 930 & 0.595 & 0.000 & 0.000 & 0.000 & 0.039 & 0.570 & 0.000 & 0.983 & 0.991 & 0.890\\
 931 & 0.562 & 0.000 & 0.000 & 0.000 & 0.028 & 0.543 & 0.000 & 0.983 & 0.991 & 0.849\\
 932 & 0.516 & 0.000 & 0.000 & 0.000 & 0.019 & 0.501 & 0.000 & 0.983 & 0.991 & 0.788\\
 933 & 0.499 & 0.000 & 0.000 & 0.000 & 0.014 & 0.486 & 0.000 & 0.983 & 0.991 & 0.771\\
 934 & 0.445 & 0.000 & 0.000 & 0.000 & 0.010 & 0.435 & 0.000 & 0.984 & 0.991 & 0.696\\
 935 & 0.473 & 0.000 & 0.000 & 0.000 & 0.008 & 0.464 & 0.000 & 0.984 & 0.991 & 0.751\\
 936 & 0.409 & 0.000 & 0.000 & 0.000 & 0.006 & 0.401 & 0.000 & 0.984 & 0.991 & 0.657\\
 937 & 0.442 & 0.000 & 0.000 & 0.000 & 0.005 & 0.435 & 0.000 & 0.984 & 0.991 & 0.720\\
 938 & 0.447 & 0.000 & 0.000 & 0.000 & 0.004 & 0.441 & 0.000 & 0.984 & 0.991 & 0.739\\
 939 & 0.520 & 0.000 & 0.000 & 0.000 & 0.004 & 0.513 & 0.000 & 0.984 & 0.991 & 0.870\\
 940 & 0.536 & 0.000 & 0.000 & 0.000 & 0.004 & 0.529 & 0.000 & 0.984 & 0.991 & 0.910\\
 941 & 0.504 & 0.000 & 0.000 & 0.000 & 0.003 & 0.498 & 0.000 & 0.984 & 0.991 & 0.868\\
 942 & 0.505 & 0.000 & 0.000 & 0.000 & 0.002 & 0.499 & 0.000 & 0.984 & 0.991 & 0.883\\
 943 & 0.437 & 0.000 & 0.000 & 0.000 & 0.002 & 0.431 & 0.000 & 0.984 & 0.991 & 0.774\\
 944 & 0.425 & 0.000 & 0.000 & 0.000 & 0.002 & 0.419 & 0.000 & 0.984 & 0.991 & 0.763\\
 945 & 0.478 & 0.000 & 0.000 & 0.000 & 0.001 & 0.471 & 0.000 & 0.984 & 0.991 & 0.868\\
 946 & 0.393 & 0.000 & 0.000 & 0.000 & 0.001 & 0.386 & 0.000 & 0.984 & 0.991 & 0.722\\
 947 & 0.468 & 0.000 & 0.000 & 0.000 & 0.001 & 0.459 & 0.000 & 0.984 & 0.991 & 0.868\\
 948 & 0.412 & 0.000 & 0.000 & 0.000 & 0.001 & 0.404 & 0.000 & 0.984 & 0.991 & 0.773\\
 949 & 0.498 & 0.000 & 0.000 & 0.000 & 0.001 & 0.487 & 0.000 & 0.984 & 0.991 & 0.943\\
 950 & 0.358 & 0.000 & 0.000 & 0.000 & 0.000 & 0.349 & 0.000 & 0.984 & 0.991 & 0.685\\
 951 & 0.493 & 0.000 & 0.000 & 0.000 & 0.001 & 0.480 & 0.000 & 0.984 & 0.992 & 0.952\\
 952 & 0.397 & 0.000 & 0.000 & 0.000 & 0.000 & 0.386 & 0.000 & 0.984 & 0.992 & 0.775\\
 953 & 0.435 & 0.000 & 0.000 & 0.000 & 0.000 & 0.422 & 0.000 & 0.984 & 0.992 & 0.858\\
 954 & 0.448 & 0.000 & 0.000 & 0.000 & 0.000 & 0.435 & 0.000 & 0.984 & 0.992 & 0.895\\
 955 & 0.426 & 0.000 & 0.000 & 0.000 & 0.000 & 0.413 & 0.000 & 0.984 & 0.992 & 0.860\\
 956 & 0.415 & 0.000 & 0.000 & 0.000 & 0.000 & 0.402 & 0.000 & 0.984 & 0.992 & 0.847\\
 957 & 0.400 & 0.000 & 0.000 & 0.000 & 0.000 & 0.388 & 0.000 & 0.984 & 0.992 & 0.827\\
 958 & 0.425 & 0.000 & 0.000 & 0.000 & 0.000 & 0.412 & 0.000 & 0.984 & 0.992 & 0.889\\
 959 & 0.409 & 0.000 & 0.000 & 0.000 & 0.000 & 0.395 & 0.000 & 0.984 & 0.992 & 0.866\\
 960 & 0.414 & 0.000 & 0.000 & 0.000 & 0.000 & 0.401 & 0.000 & 0.984 & 0.992 & 0.889\\
 961 & 0.414 & 0.000 & 0.000 & 0.000 & 0.000 & 0.401 & 0.000 & 0.984 & 0.992 & 0.900\\
 962 & 0.407 & 0.000 & 0.000 & 0.000 & 0.000 & 0.394 & 0.000 & 0.984 & 0.992 & 0.895\\
 963 & 0.412 & 0.000 & 0.000 & 0.000 & 0.000 & 0.399 & 0.000 & 0.984 & 0.992 & 0.920\\
 964 & 0.399 & 0.000 & 0.000 & 0.000 & 0.000 & 0.386 & 0.000 & 0.984 & 0.992 & 0.904\\
 965 & 0.399 & 0.000 & 0.000 & 0.000 & 0.000 & 0.387 & 0.000 & 0.984 & 0.992 & 0.918\\
 966 & 0.394 & 0.000 & 0.000 & 0.000 & 0.000 & 0.382 & 0.000 & 0.984 & 0.992 & 0.920\\
 967 & 0.393 & 0.000 & 0.000 & 0.000 & 0.000 & 0.381 & 0.000 & 0.984 & 0.992 & 0.931\\
 968 & 0.400 & 0.000 & 0.000 & 0.000 & 0.000 & 0.388 & 0.000 & 0.985 & 0.992 & 0.962\\
 969 & 0.402 & 0.000 & 0.000 & 0.000 & 0.000 & 0.390 & 0.000 & 0.985 & 0.992 & 0.982\\
 970 & 0.390 & 0.000 & 0.000 & 0.000 & 0.000 & 0.378 & 0.000 & 0.985 & 0.992 & 0.967\\
 971 & 0.391 & 0.000 & 0.000 & 0.000 & 0.000 & 0.380 & 0.000 & 0.985 & 0.992 & 0.988\\
 972 & 0.379 & 0.000 & 0.000 & 0.000 & 0.000 & 0.368 & 0.000 & 0.985 & 0.992 & 0.974\\
 973 & 0.368 & 0.000 & 0.000 & 0.000 & 0.000 & 0.358 & 0.000 & 0.985 & 0.992 & 0.963\\
 974 & 0.358 & 0.000 & 0.000 & 0.000 & 0.000 & 0.349 & 0.000 & 0.985 & 0.992 & 0.955\\
 975 & 0.349 & 0.000 & 0.000 & 0.000 & 0.000 & 0.341 & 0.000 & 0.985 & 0.992 & 0.947\\
 976 & 0.345 & 0.000 & 0.000 & 0.000 & 0.000 & 0.337 & 0.000 & 0.985 & 0.992 & 0.953\\
 977 & 0.343 & 0.000 & 0.000 & 0.000 & 0.000 & 0.335 & 0.000 & 0.985 & 0.992 & 0.966\\
 978 & 0.335 & 0.000 & 0.000 & 0.000 & 0.000 & 0.327 & 0.000 & 0.985 & 0.992 & 0.962\\
 979 & 0.334 & 0.000 & 0.000 & 0.000 & 0.000 & 0.326 & 0.000 & 0.985 & 0.992 & 0.975\\
 980 & 0.323 & 0.000 & 0.000 & 0.000 & 0.000 & 0.315 & 0.000 & 0.985 & 0.993 & 0.961\\
 981 & 0.325 & 0.000 & 0.000 & 0.000 & 0.000 & 0.318 & 0.000 & 0.985 & 0.993 & 0.989\\
 982 & 0.318 & 0.000 & 0.000 & 0.000 & 0.000 & 0.311 & 0.000 & 0.985 & 0.993 & 0.987\\
 983 & 0.308 & 0.000 & 0.000 & 0.000 & 0.000 & 0.302 & 0.000 & 0.985 & 0.993 & 0.978\\
 984 & 0.307 & 0.000 & 0.000 & 0.000 & 0.000 & 0.301 & 0.000 & 0.985 & 0.993 & 0.997\\
 985 & 0.298 & 0.000 & 0.000 & 0.000 & 0.000 & 0.292 & 0.000 & 0.985 & 0.993 & 0.984\\
 986 & 0.295 & 0.000 & 0.000 & 0.000 & 0.000 & 0.290 & 0.000 & 0.985 & 0.993 & 0.998\\
 987 & 0.287 & 0.000 & 0.000 & 0.000 & 0.000 & 0.282 & 0.000 & 0.985 & 0.993 & 0.996\\
 988 & 0.278 & 0.000 & 0.000 & 0.000 & 0.000 & 0.274 & 0.000 & 0.985 & 0.993 & 0.995\\
 989 & 0.272 & 0.000 & 0.000 & 0.000 & 0.000 & 0.268 & 0.000 & 0.985 & 0.993 & 0.999\\
 990 & 0.264 & 0.000 & 0.000 & 0.000 & 0.000 & 0.260 & 0.000 & 0.985 & 0.993 & 0.996\\
 991 & 0.259 & 0.000 & 0.000 & 0.000 & 0.000 & 0.255 & 0.000 & 0.985 & 0.993 & 0.998\\
 992 & 0.253 & 0.000 & 0.000 & 0.000 & 0.000 & 0.250 & 0.000 & 0.985 & 0.993 & 0.998\\
 993 & 0.246 & 0.000 & 0.000 & 0.000 & 0.000 & 0.243 & 0.000 & 0.985 & 0.993 & 0.997\\
 994 & 0.241 & 0.000 & 0.000 & 0.000 & 0.000 & 0.238 & 0.000 & 0.985 & 0.993 & 0.999\\
 995 & 0.235 & 0.000 & 0.000 & 0.000 & 0.000 & 0.232 & 0.000 & 0.985 & 0.993 & 0.999\\
 996 & 0.229 & 0.000 & 0.000 & 0.000 & 0.000 & 0.227 & 0.000 & 0.985 & 0.993 & 0.999\\
 997 & 0.224 & 0.000 & 0.000 & 0.000 & 0.000 & 0.221 & 0.000 & 0.985 & 0.993 & 0.999\\
 998 & 0.218 & 0.000 & 0.000 & 0.000 & 0.000 & 0.216 & 0.000 & 0.985 & 0.993 & 0.999\\
 999 & 0.213 & 0.000 & 0.000 & 0.000 & 0.000 & 0.211 & 0.000 & 0.985 & 0.993 & 0.999\\
1000 & 0.208 & 0.000 & 0.000 & 0.000 & 0.000 & 0.205 & 0.000 & 0.985 & 0.993 & 0.999\\
1001 & 0.203 & 0.000 & 0.000 & 0.000 & 0.000 & 0.200 & 0.000 & 0.985 & 0.993 & 0.999\\
1002 & 0.197 & 0.000 & 0.000 & 0.000 & 0.000 & 0.195 & 0.000 & 0.985 & 0.993 & 0.997\\
1003 & 0.192 & 0.000 & 0.000 & 0.000 & 0.000 & 0.189 & 0.000 & 0.985 & 0.993 & 0.999\\
1004 & 0.186 & 0.000 & 0.000 & 0.000 & 0.000 & 0.183 & 0.000 & 0.985 & 0.993 & 0.999\\
1005 & 0.181 & 0.000 & 0.000 & 0.000 & 0.000 & 0.178 & 0.000 & 0.985 & 0.993 & 1.000\\
1006 & 0.176 & 0.000 & 0.000 & 0.000 & 0.000 & 0.173 & 0.000 & 0.986 & 0.993 & 0.999\\
1007 & 0.171 & 0.000 & 0.000 & 0.000 & 0.000 & 0.168 & 0.000 & 0.986 & 0.993 & 0.999\\
1008 & 0.165 & 0.000 & 0.000 & 0.000 & 0.000 & 0.162 & 0.000 & 0.986 & 0.993 & 0.999\\
1009 & 0.160 & 0.000 & 0.000 & 0.000 & 0.000 & 0.157 & 0.000 & 0.986 & 0.993 & 0.998\\
1010 & 0.155 & 0.000 & 0.000 & 0.000 & 0.000 & 0.152 & 0.000 & 0.986 & 0.993 & 0.998\\
1011 & 0.149 & 0.000 & 0.000 & 0.000 & 0.000 & 0.147 & 0.000 & 0.986 & 0.993 & 0.999\\
1012 & 0.143 & 0.000 & 0.000 & 0.000 & 0.000 & 0.141 & 0.000 & 0.986 & 0.993 & 0.999\\
1013 & 0.138 & 0.000 & 0.000 & 0.000 & 0.000 & 0.136 & 0.000 & 0.986 & 0.993 & 1.000\\
1014 & 0.133 & 0.000 & 0.000 & 0.000 & 0.000 & 0.131 & 0.000 & 0.986 & 0.993 & 1.000\\
1015 & 0.129 & 0.000 & 0.000 & 0.000 & 0.000 & 0.127 & 0.000 & 0.986 & 0.993 & 0.999\\
1016 & 0.126 & 0.000 & 0.000 & 0.000 & 0.000 & 0.124 & 0.000 & 0.986 & 0.994 & 0.999\\
1017 & 0.122 & 0.000 & 0.000 & 0.000 & 0.000 & 0.120 & 0.000 & 0.986 & 0.993 & 0.999\\
1018 & 0.118 & 0.000 & 0.000 & 0.000 & 0.000 & 0.116 & 0.000 & 0.986 & 0.994 & 0.999\\
1019 & 0.113 & 0.000 & 0.000 & 0.000 & 0.000 & 0.111 & 0.000 & 0.986 & 0.994 & 0.999\\
1020 & 0.108 & 0.000 & 0.000 & 0.000 & 0.000 & 0.106 & 0.000 & 0.986 & 0.994 & 1.000\\
1021 & 0.103 & 0.000 & 0.000 & 0.000 & 0.000 & 0.102 & 0.000 & 0.986 & 0.994 & 1.000\\
1022 & 0.098 & 0.000 & 0.000 & 0.000 & 0.000 & 0.097 & 0.000 & 0.986 & 0.994 & 0.999\\
1023 & 0.095 & 0.000 & 0.000 & 0.000 & 0.000 & 0.094 & 0.000 & 0.986 & 0.994 & 0.999\\
1024 & 0.092 & 0.000 & 0.000 & 0.000 & 0.000 & 0.091 & 0.000 & 0.986 & 0.994 & 0.998\\
1025 & 0.089 & 0.000 & 0.000 & 0.000 & 0.000 & 0.088 & 0.000 & 0.986 & 0.994 & 1.000\\
1026 & 0.085 & 0.000 & 0.000 & 0.000 & 0.000 & 0.084 & 0.000 & 0.986 & 0.994 & 0.999\\
1027 & 0.082 & 0.000 & 0.000 & 0.000 & 0.000 & 0.081 & 0.000 & 0.986 & 0.994 & 0.999\\
1028 & 0.079 & 0.000 & 0.000 & 0.000 & 0.000 & 0.078 & 0.000 & 0.986 & 0.994 & 0.999\\
1029 & 0.076 & 0.000 & 0.000 & 0.000 & 0.000 & 0.075 & 0.000 & 0.986 & 0.994 & 0.999\\
1030 & 0.072 & 0.000 & 0.000 & 0.000 & 0.000 & 0.071 & 0.000 & 0.986 & 0.994 & 1.000\\
1031 & 0.068 & 0.000 & 0.000 & 0.000 & 0.000 & 0.067 & 0.000 & 0.986 & 0.994 & 0.999\\
1032 & 0.065 & 0.000 & 0.000 & 0.000 & 0.000 & 0.064 & 0.000 & 0.986 & 0.994 & 1.000\\
1033 & 0.061 & 0.000 & 0.000 & 0.000 & 0.000 & 0.060 & 0.000 & 0.986 & 0.994 & 1.000\\
1034 & 0.058 & 0.000 & 0.000 & 0.000 & 0.000 & 0.057 & 0.000 & 0.986 & 0.994 & 1.000\\
1035 & 0.056 & 0.000 & 0.000 & 0.000 & 0.000 & 0.055 & 0.000 & 0.986 & 0.994 & 1.000\\
1036 & 0.053 & 0.000 & 0.000 & 0.000 & 0.000 & 0.053 & 0.000 & 0.986 & 0.994 & 0.999\\
1037 & 0.051 & 0.000 & 0.000 & 0.000 & 0.000 & 0.050 & 0.000 & 0.986 & 0.994 & 0.999\\
1038 & 0.049 & 0.000 & 0.000 & 0.000 & 0.000 & 0.048 & 0.000 & 0.986 & 0.994 & 0.999\\
1039 & 0.046 & 0.000 & 0.000 & 0.000 & 0.000 & 0.045 & 0.000 & 0.986 & 0.994 & 0.999\\
1040 & 0.044 & 0.000 & 0.000 & 0.000 & 0.000 & 0.043 & 0.000 & 0.986 & 0.994 & 0.999\\
1041 & 0.042 & 0.000 & 0.000 & 0.000 & 0.000 & 0.041 & 0.000 & 0.986 & 0.994 & 0.999\\
1042 & 0.040 & 0.000 & 0.000 & 0.000 & 0.000 & 0.039 & 0.000 & 0.986 & 0.994 & 0.999\\
1043 & 0.038 & 0.000 & 0.000 & 0.000 & 0.000 & 0.037 & 0.000 & 0.986 & 0.994 & 0.999\\
1044 & 0.037 & 0.000 & 0.000 & 0.000 & 0.000 & 0.036 & 0.000 & 0.986 & 0.994 & 0.999\\
1045 & 0.036 & 0.000 & 0.000 & 0.000 & 0.000 & 0.035 & 0.000 & 0.986 & 0.994 & 0.999\\
1046 & 0.035 & 0.000 & 0.000 & 0.000 & 0.000 & 0.034 & 0.000 & 0.986 & 0.994 & 0.999\\
1047 & 0.034 & 0.000 & 0.000 & 0.000 & 0.000 & 0.033 & 0.000 & 0.986 & 0.994 & 0.999\\
1048 & 0.032 & 0.000 & 0.000 & 0.000 & 0.000 & 0.032 & 0.000 & 0.987 & 0.994 & 0.998\\
1049 & 0.031 & 0.000 & 0.000 & 0.000 & 0.000 & 0.030 & 0.000 & 0.987 & 0.994 & 0.998\\
1050 & 0.029 & 0.000 & 0.000 & 0.000 & 0.000 & 0.029 & 0.000 & 0.987 & 0.994 & 0.998\\
1051 & 0.028 & 0.000 & 0.000 & 0.000 & 0.000 & 0.028 & 0.000 & 0.987 & 0.994 & 0.998\\
1052 & 0.027 & 0.000 & 0.000 & 0.000 & 0.000 & 0.027 & 0.000 & 0.987 & 0.994 & 0.997\\
1053 & 0.026 & 0.000 & 0.000 & 0.000 & 0.000 & 0.026 & 0.000 & 0.987 & 0.994 & 0.997\\
1054 & 0.025 & 0.000 & 0.000 & 0.000 & 0.000 & 0.025 & 0.000 & 0.987 & 0.994 & 0.996\\
1055 & 0.024 & 0.000 & 0.000 & 0.000 & 0.000 & 0.024 & 0.000 & 0.987 & 0.994 & 0.996\\
1056 & 0.023 & 0.000 & 0.000 & 0.000 & 0.000 & 0.023 & 0.000 & 0.987 & 0.994 & 0.995\\
1057 & 0.022 & 0.000 & 0.000 & 0.000 & 0.000 & 0.022 & 0.000 & 0.987 & 0.994 & 0.994\\
1058 & 0.022 & 0.000 & 0.000 & 0.000 & 0.000 & 0.021 & 0.000 & 0.987 & 0.994 & 0.994\\
1059 & 0.020 & 0.000 & 0.000 & 0.000 & 0.000 & 0.020 & 0.000 & 0.987 & 0.994 & 0.993\\
1060 & 0.019 & 0.000 & 0.000 & 0.000 & 0.000 & 0.019 & 0.000 & 0.987 & 0.995 & 0.992\\
1061 & 0.018 & 0.000 & 0.000 & 0.000 & 0.000 & 0.018 & 0.000 & 0.987 & 0.995 & 0.992\\
1062 & 0.017 & 0.000 & 0.000 & 0.000 & 0.000 & 0.017 & 0.000 & 0.987 & 0.995 & 0.991\\
1063 & 0.017 & 0.000 & 0.000 & 0.000 & 0.000 & 0.016 & 0.000 & 0.987 & 0.995 & 0.991\\
1064 & 0.016 & 0.000 & 0.000 & 0.000 & 0.000 & 0.015 & 0.000 & 0.987 & 0.995 & 0.990\\
1065 & 0.015 & 0.000 & 0.000 & 0.000 & 0.000 & 0.015 & 0.000 & 0.987 & 0.995 & 0.989\\
1066 & 0.015 & 0.000 & 0.000 & 0.000 & 0.000 & 0.014 & 0.000 & 0.987 & 0.995 & 0.989\\
1067 & 0.014 & 0.000 & 0.000 & 0.000 & 0.000 & 0.014 & 0.000 & 0.987 & 0.995 & 0.990\\
1068 & 0.014 & 0.000 & 0.000 & 0.000 & 0.000 & 0.013 & 0.000 & 0.987 & 0.995 & 0.989\\
1069 & 0.013 & 0.000 & 0.000 & 0.000 & 0.000 & 0.012 & 0.000 & 0.987 & 0.995 & 0.991\\
1070 & 0.012 & 0.000 & 0.000 & 0.000 & 0.000 & 0.012 & 0.000 & 0.987 & 0.995 & 0.992\\
1071 & 0.012 & 0.000 & 0.000 & 0.000 & 0.000 & 0.011 & 0.000 & 0.987 & 0.995 & 0.994\\
1072 & 0.011 & 0.000 & 0.000 & 0.000 & 0.000 & 0.011 & 0.000 & 0.987 & 0.995 & 0.994\\
1073 & 0.011 & 0.000 & 0.000 & 0.000 & 0.000 & 0.011 & 0.000 & 0.987 & 0.995 & 0.995\\
1074 & 0.011 & 0.000 & 0.000 & 0.000 & 0.000 & 0.010 & 0.000 & 0.987 & 0.995 & 0.997\\
1075 & 0.010 & 0.000 & 0.000 & 0.000 & 0.000 & 0.010 & 0.000 & 0.987 & 0.995 & 0.994\\
1076 & 0.009 & 0.000 & 0.000 & 0.000 & 0.000 & 0.009 & 0.000 & 0.987 & 0.995 & 0.997\\
1077 & 0.009 & 0.000 & 0.000 & 0.000 & 0.000 & 0.009 & 0.000 & 0.987 & 0.995 & 0.995\\
1078 & 0.008 & 0.000 & 0.000 & 0.000 & 0.000 & 0.008 & 0.000 & 0.987 & 0.995 & 0.996\\
1079 & 0.008 & 0.000 & 0.000 & 0.000 & 0.000 & 0.008 & 0.000 & 0.987 & 0.995 & 0.998\\
1080 & 0.008 & 0.000 & 0.000 & 0.000 & 0.000 & 0.008 & 0.000 & 0.987 & 0.995 & 0.994\\
1081 & 0.007 & 0.000 & 0.000 & 0.000 & 0.000 & 0.007 & 0.000 & 0.987 & 0.995 & 0.994\\
1082 & 0.007 & 0.000 & 0.000 & 0.000 & 0.000 & 0.007 & 0.000 & 0.987 & 0.995 & 0.998\\
1083 & 0.007 & 0.000 & 0.000 & 0.000 & 0.000 & 0.007 & 0.000 & 0.987 & 0.995 & 0.999\\
1084 & 0.006 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.000 & 0.987 & 0.995 & 0.991\\
1085 & 0.006 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.000 & 0.987 & 0.995 & 0.996\\
1086 & 0.006 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.000 & 0.987 & 0.995 & 0.985\\
1087 & 0.006 & 0.000 & 0.000 & 0.000 & 0.000 & 0.006 & 0.000 & 0.987 & 0.995 & 0.995\\
1088 & 0.006 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.000 & 0.987 & 0.995 & 0.997\\
1089 & 0.005 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.000 & 0.988 & 0.995 & 0.995\\
1090 & 0.005 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.000 & 0.988 & 0.995 & 0.987\\
1091 & 0.005 & 0.000 & 0.000 & 0.000 & 0.000 & 0.005 & 0.000 & 0.988 & 0.995 & 0.996\\
1092 & 0.004 & 0.000 & 0.000 & 0.000 & 0.000 & 0.004 & 0.000 & 0.988 & 0.995 & 0.998\\
1093 & 0.004 & 0.000 & 0.000 & 0.000 & 0.000 & 0.004 & 0.000 & 0.988 & 0.995 & 0.978\\
1094 & 0.004 & 0.000 & 0.000 & 0.000 & 0.000 & 0.004 & 0.000 & 0.988 & 0.995 & 0.995\\
1095 & 0.004 & 0.000 & 0.000 & 0.000 & 0.000 & 0.004 & 0.000 & 0.988 & 0.995 & 0.985\\
1096 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.988 & 0.995 & 0.981\\
1097 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.988 & 0.995 & 0.998\\
1098 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.988 & 0.995 & 0.981\\
1099 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.003 & 0.000 & 0.988 & 0.995 & 0.983\\
1100 & 0.003 & 0.000 & 0.000 & 0.000 & 0.000 & 0.002 & 0.000 & 0.988 & 0.995 & 0.972\\
\enddata
\tablecomments{The columns are wavelength [nm] and capture
  cross-section [m$^2$-e$^-$/photon] for each of the \PS\ bandpasses,
  {\it including} the nominal 1.2 airmasses of atmospheric extinction.
  The last three columns list the transmission of the \PS\ standard
  atmosphere from aerosol scattering, Rayleigh scattering, and
  molecular absorption.}
\label{tab:bandpass}
\end{deluxetable}

